Estimation of Propagated Risk in LLM-based Multi-Agent Systems

Large Language Model (LLM) based multi-agent systems introduce a distinctive reliability challenge in which actions taken by upstream agents can affect the correctness of downstream agents. While prior work has investigated error propagation and developed methods for estimating uncertainty inherited from upstream agents, existing approaches do not explicitly model how realized sender-receiver interactions contribute to downstream error risk under different sender correctness states. In this work, we study agent-level error-risk estimation from multi-agent execution traces. We propose Interaction-Effect Propagation (IE-Prop), an interaction-conditioned model that learns separate effects for correct and incorrect upstream agents. For each sender-receiver interaction, the model combines these conditional effects using the sender's estimated error risk, and recursively propagates the resulting risk estimates through the execution graph. We evaluate our approach across three multi-agent architectures and three benchmarks. Across all evaluated architectures, our approach raises the final-node AUROC over the established baseline by approximately 0.05 points on average. Furthermore, tracking risk across multiple agent steps contributes a distinct +0.03 AUROC gain in sequential systems. These results show that realized inter-agent interactions provide predictive information beyond receiver-local evidence, while the value of multi-step risk tracking depends on the system's information-flow structure.

==> tables/agentic_full.tex <==
\begin{table*}[t]
\centering\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{WebArena} & \multicolumn{3}{c}{AppWorld} & \multicolumn{3}{c}{AppWorld, both trial seeds} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Method & NLL & Brier & AUROC & NLL & Brier & AUROC & NLL & Brier & AUROC \\
\midrule
Receiver Only & \textbf{0.442} & 0.147 & 0.766 & \textbf{0.592} & \textbf{0.201} & \textbf{0.634} & \textbf{0.562} & \textbf{0.188} & \textbf{0.674} \\
Learned noisy-OR (contamination) & 0.670 & 0.211 & 0.560 & 0.617 & 0.212 & 0.606 & 0.610 & 0.209 & 0.630 \\
Interaction without parent state & 1.034 & 0.233 & 0.426 & 0.643 & 0.220 & 0.572 & 0.638 & 0.216 & 0.613 \\
IE propagation, recursive-soft & 0.947 & 0.232 & 0.434 & 0.643 & 0.220 & 0.572 & 0.634 & 0.215 & 0.612 \\
IE propagation, recursive-soft, linear head & 0.568 & 0.185 & 0.620 & 0.614 & 0.209 & 0.598 & 0.612 & 0.208 & 0.630 \\
IE effects with PME inference, recursive-soft & 0.938 & 0.231 & 0.435 & 0.643 & 0.220 & 0.572 & 0.634 & 0.215 & 0.612 \\
IE propagation, state-supervised & 0.463 & 0.148 & \textbf{0.835} & 0.634 & 0.218 & 0.616 & 0.608 & 0.208 & 0.660 \\
\quad same potentials, PME inference & 0.458 & \textbf{0.146} & 0.815 & 0.607 & 0.210 & 0.618 & 0.580 & 0.199 & 0.663 \\
\quad same potentials, learned parent joint & 0.526 & 0.176 & 0.663 & 0.618 & 0.211 & 0.603 & 0.590 & 0.201 & 0.640 \\
\textit{Oracle parent states (analysis only)} & 0.333 & 0.099 & 0.889 & 0.488 & 0.149 & 0.801 & 0.483 & 0.146 & 0.796 \\
\bottomrule
\end{tabular}}
\caption{All executor-risk models. The last block is an extension of AppWorld whose analysis plan was fixed before data collection, with both trial seeds ($n{=}719$ trajectories, same 136 tasks). The linear head replaces the edge MLP; the learned parent joint is a pairwise Ising model over the executor's parents fitted on the same potentials. Bold: best value in each column (oracle excluded).}
\label{tab:agenticfull}
\end{table*}


==> tables/agentic_main.tex <==
\begin{table*}[t]
\centering\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{WebArena ($n{=}447$ trajectories)} & \multicolumn{3}{c}{AppWorld ($n{=}350$ trajectories)} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Executor error risk & NLL & Brier & AUROC & NLL & Brier & AUROC \\
\midrule
Receiver Only & \textbf{0.442} & 0.147 & 0.766 & \textbf{0.592} & \textbf{0.201} & \textbf{0.634} \\
Learned noisy-OR (contamination) & 0.670 & 0.211 & 0.560 & 0.617 & 0.212 & 0.606 \\
Interaction without parent state & 1.034 & 0.233 & 0.426 & 0.643 & 0.220 & 0.572 \\
IE propagation, recursive-soft & 0.947 & 0.232 & 0.434 & 0.643 & 0.220 & 0.572 \\
IE propagation, state-supervised & 0.463 & 0.148 & \textbf{0.835} & 0.634 & 0.218 & 0.616 \\
\quad same potentials, PME inference & 0.458 & \textbf{0.146} & 0.815 & 0.607 & 0.210 & 0.618 \\
\midrule
\textit{Oracle parent states (analysis only)} & 0.333 & 0.099 & 0.889 & 0.488 & 0.149 & 0.801 \\
\bottomrule
\end{tabular}
\caption{Error risk of the final executor (out-of-fold, seed-averaged; IE: interaction-effect). All learned rows share the frozen edge embedding, nested grouped cross-validation and receiver head. Recursive-soft rows are trained through the propagation rule; the state-supervised row is fitted with observed parent states and deployed with estimated parent risks (Appendix~\ref{app:agentictrain}). The learned noisy-OR replaces the two effects by a transmission probability $\alpha_{pv}$ computed from the same interaction embedding. The oracle feeds the true parent states into the state-supervised potentials and is not deployable. WebArena, state-supervised IE propagation $-$ Receiver Only (task-clustered 95\% CI): $\Delta$NLL +0.020 [$-$0.099, 0.134], $\Delta$Brier +0.001 [$-$0.045, 0.044], $\Delta$AUROC +0.069 [$-$0.009, 0.139]. Bold: best value in each column (oracle excluded).}
\label{tab:agentic}
\end{table*}


==> tables/appworld_revised.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{lcc}
\toprule
AppWorld, supervised node risks & NLL & AUROC \\
\midrule
Receiver Only (local readout) & \textbf{0.592} & \textbf{0.634} \\
IE propagation, text effects & 0.678 & 0.502 \\
IE effects with PME inference, text & 0.633 & 0.505 \\
IE propagation, role-pair effects & 0.693 & 0.536 \\
Oracle, text effects & 0.460 & 0.835 \\
Oracle, role-pair effects & 0.417 & 0.848 \\
\bottomrule
\end{tabular}}
\caption{AppWorld with supervised node-risk models (parent AUROC: source 0.46$\to$0.71, specialists 0.60$\to$0.70) and state-supervised effects with a linear text head or six role-pair scalars. Better parent risks add +0.007 [$-$0.007, 0.021] nats beyond the receiver's evidence. Bold: best value in each column (oracles excluded).}
\label{tab:appworldrev}
\end{table}


==> tables/bottleneck.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{lcc}
\toprule
 & WebArena & AppWorld \\
\midrule
Parent-risk AUROC & 0.59 (H) & 0.62 (A), 0.47 (S) \\
\addlinespace[2pt]\multicolumn{3}{l}{\emph{NLL gain over receiver-local evidence (nats)}} \\
\quad + deployable $\hat r_{\mathrm{Pa}}$ & +0.064 [0.014, 0.124] & +0.007 [$-$0.011, 0.025] \\
\quad + parent-local $\sigma(b_p)$ & $-$0.005 [$-$0.026, 0.017] & +0.015 [$-$0.004, 0.033] \\
\quad + true $E_{\mathrm{Pa}}$ (oracle) & +0.082 [0.027, 0.134] & +0.241 [0.162, 0.321] \\
\addlinespace[2pt]\multicolumn{3}{l}{\emph{State-supervised, NLL with $r_p=(1-\varepsilon)\hat r_p+\varepsilon E_p$}} \\
\quad $\varepsilon=0$ & 0.463 & 0.634 \\
\quad $\varepsilon=0.25$ & 0.389 & 0.581 \\
\quad $\varepsilon=1$ & 0.333 & 0.488 \\
\quad Receiver Only & 0.442 & 0.592 \\
\bottomrule
\end{tabular}}
\caption{Upstream-information diagnostics at the executor. Parent-risk AUROC: the deployable propagated risks of the executor's parents against their true error, by role. Gains: out-of-fold L2 logistic regressions of executor error on the receiver's local evidence, plus the deployable parent risks or the true parent states (task-clustered 95\% CI); $\hat r_{\mathrm{Pa}}$ are the propagated risks the deployed model uses, and $\sigma(b_p)$ are the parents' own receiver-only risks. Last block: the same state-supervised potentials fed increasingly accurate parent states.}
\label{tab:bottleneck}
\end{table}


==> tables/branch_sep.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\toprule
 & \multicolumn{2}{c}{Recursive-soft} & State-sup. \\
\cmidrule(lr){2-3}\cmidrule(lr){4-4}
System & med.\ $|\Delta|$ & $|\Delta|{<}0.1$ & med.\ $|\Delta|$ \\
\midrule
AppWorld & 0.027 & 0.98 & 1.35 \\
WebArena & 0.095 & 0.52 & 1.98 \\
\bottomrule
\end{tabular}
\caption{Branch separation $\Delta_{pv}=\delta^{(1)}_{pv}-\delta^{(0)}_{pv}$ on the edges into the scored node (all edges). $|\Delta|{<}0.1$: fraction of edges whose two effects nearly coincide. The QA counterparts are in Table~\ref{tab:qabranch}. With supervised AppWorld node risks the state-supervised median is 1.52 (Appendix~\ref{app:appworld}).}
\label{tab:branch}
\end{table}


==> tables/data.tex <==
\begin{table}[t]
\centering\footnotesize
\begin{tabular}{llr}
\toprule
System & Source (model) & Train traces \\
\midrule
sequential & gsm8k (0.6B) & 1{,}223 \\
sequential & gsm8k (1.7B) & 5{,}736 \\
sequential & gsm8k (4B) & 7{,}448 \\
sequential & medqa (0.6B) & 1{,}743 \\
sequential & medqa (1.7B) & 10{,}125 \\
sequential & medqa (4B) & 10{,}119 \\
sequential & webqa (0.6B) & 9{,}284 \\
sequential & webqa (1.7B) & 16{,}231 \\
sequential & webqa (4B) & 16{,}085 \\
\midrule
fully connected & gsm8k (0.6B) & 6{,}486 \\
fully connected & gsm8k (1.7B) & 7{,}375 \\
fully connected & gsm8k (4B) & 7{,}453 \\
fully connected & medqa (0.6B) & 9{,}667 \\
fully connected & medqa (1.7B) & 10{,}165 \\
fully connected & medqa (4B) & 10{,}172 \\
fully connected & webqa (0.6B) & 17{,}386 \\
fully connected & webqa (1.7B) & 17{,}419 \\
fully connected & webqa (4B) & 17{,}656 \\
\midrule
hierarchy & gsm8k (0.6B) & 558 \\
hierarchy & gsm8k (1.7B) & 243 \\
hierarchy & gsm8k (4B) & 6{,}540 \\
hierarchy & medqa (0.6B) & 153 \\
hierarchy & medqa (1.7B) & 1{,}483 \\
hierarchy & medqa (4B) & 4{,}841 \\
\bottomrule
\end{tabular}
\caption{Training traces per source after dropping traces with an unlabeled node (Appendix~\ref{app:qa}). Training and test traces are labeled by the same procedure.}
\label{tab:data}
\end{table}


==> tables/dependence.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{4}{c}{WebArena} & \multicolumn{4}{c}{AppWorld} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
Quartile & $|$corr$|$ & Var$(Z)$ & NP & PME & $|$corr$|$ & Var$(Z)$ & NP & PME \\
\midrule
Q1 & 0.124 & 0.945 & 0.029 & 0.002 & 0.239 & 1.149 & 0.035 & 0.008 \\
Q2 & 0.175 & 0.765 & 0.031 & 0.002 & 0.282 & 1.510 & 0.050 & 0.012 \\
Q3 & 0.221 & 1.531 & 0.044 & 0.006 & 0.308 & 1.759 & 0.053 & 0.013 \\
Q4 & 0.289 & 3.903 & 0.093 & 0.015 & 0.348 & 2.106 & 0.066 & 0.018 \\
\bottomrule
\end{tabular}}
\caption{Executor approximation error by quartile of induced parent dependence (maximum absolute correlation among the executor's parents in the network induced by the state-supervised potentials).}
\label{tab:dependence}
\end{table}


==> tables/fidelity.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{lcc}
\toprule
State-supervised potentials & WebArena & AppWorld \\
\midrule
NP error, mean / p95 / max & 0.049 / 0.187 / 0.362 & 0.051 / 0.078 / 0.096 \\
PME error, mean / max & 0.006 / 0.042 & 0.013 / 0.031 \\
$\rho$(NP error, $\mathrm{Var}(Z_v)$) & 0.78 & 0.73 \\
Executor AUROC, NP / PME & 0.835 / 0.815 & 0.616 / 0.618 \\
Executor $\Delta$NLL, PME $-$ NP & $-$0.005 [$-$0.056, 0.044] & $-$0.027 [$-$0.052, $-$0.006] \\
\bottomrule
\end{tabular}}
\caption{Approximation fidelity on the real executor graphs. Error: $|r_{\mathrm{exact}}-r|$, where the exact value is the executor marginal of the network induced by the learned potentials. PME: exact average under a product of parent marginals. $\rho$: Spearman correlation. Last row: task-clustered 95\% CI. Full results in Appendix~\ref{app:fidelity}.}
\label{tab:fidelity}
\end{table}


==> tables/fidelity_full.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{llcc}
\toprule
Potentials & Quantity & WebArena & AppWorld \\
\midrule
State-sup. & NP error, mean / median & 0.0493 / 0.0224 & 0.0512 / 0.0522 \\
 & NP error, p95 / max & 0.1867 / 0.3624 & 0.0781 / 0.0965 \\
 & NP local gap, mean & 0.0357 & 0.0502 \\
 & PME error, mean / max & 0.0064 / 0.0425 & 0.0127 / 0.0311 \\
 & Local bound holds & 100\% & 100\% \\
\midrule
Rec.-soft & NP error, mean / median & 0.0006 / 0.0003 & 0.0000 / 0.0000 \\
 & NP error, p95 / max & 0.0024 / 0.0042 & 0.0001 / 0.0002 \\
 & NP local gap, mean & 0.0006 & 0.0000 \\
 & PME error, mean / max & 0.0000 / 0.0000 & 0.0000 / 0.0000 \\
 & Local bound holds & 100\% & 100\% \\
\midrule
& $\rho$(NP error, $\mathrm{Var}(Z_v)$), state-sup. & 0.78 & 0.73 \\
& $\rho$(PME error, max $|$corr$|$), state-sup. & 0.65 & 0.71 \\
& Runtime per trajectory, NP / PME / exact (ms) & 0.08 / 0.15 / 0.23 & 0.05 / 0.11 / 0.13 \\
\bottomrule
\end{tabular}}
\caption{Inference fidelity at the executor for both potential sets. Local gap: NP computed from the exact parent marginals, i.e.\ the quantity bounded by Eq.~\ref{eq:bound}; the bound is checked per trajectory with the exact parent distribution.}
\label{tab:fidelityfull}
\end{table}


==> tables/free_learner.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{GSM8K} & \multicolumn{3}{c}{MedQA} & \multicolumn{3}{c}{WebQA} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
System & Verb. & MSP & Entropy & Verb. & MSP & Entropy & Verb. & MSP & Entropy \\
\midrule
Sequential & 0.680 & 0.635 & 0.636 & 0.584 & 0.593 & 0.592 & 0.640 & 0.596 & 0.597 \\
Fully connected & 0.739 & 0.738 & 0.755 & 0.578 & 0.577 & 0.595 & 0.620 & 0.598 & 0.595 \\
Hierarchy & 0.758 & 0.790 & 0.813 & 0.602 & 0.635 & 0.649 & 0.583 & 0.552 & 0.557 \\
\bottomrule
\end{tabular}%
}
\caption{AUROC of the final-node error risk for the Free Learner estimator across the three controlled system topologies in the in-domain setting. Results are averaged over the three Qwen3 model sizes and random seeds. Columns correspond to the test dataset and node uncertainty measure: verbalized confidence (Verb.), maximum sequence probability (MSP), and token entropy (Entropy).}
\label{tab:free_learner_appendix}
\end{table}

==> tables/group_ci.tex <==
\begin{table*}[p]
\centering\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{l}{\emph{In-domain}} \\
AUROC [95\% CI] & Sequential ($n{=}9$) & Fully conn. ($n{=}9$) & Hierarchy ($n{=}6$) & & \\
\midrule
PropUQ-MAS (training-free) & 0.584 [0.560, 0.607] & 0.582 [0.567, 0.597] & 0.529 [0.506, 0.554] & & \\
Raw verbalized uncertainty & 0.543 [0.525, 0.562] & 0.545 [0.533, 0.558] & 0.502 [0.481, 0.524] & & \\
Receiver Only & 0.548 [0.529, 0.567] & 0.545 [0.533, 0.558] & 0.502 [0.481, 0.523] & & \\
Receiver-text & 0.636 [0.611, 0.662] & 0.640 [0.625, 0.656] & 0.616 [0.593, 0.639] & & \\
Interaction without parent state & 0.640 [0.615, 0.667] & 0.658 [0.645, 0.673] & \textbf{0.621} [0.598, 0.645] & & \\
Free learner, local $\sigma(b_p)$ & 0.641 [0.616, 0.668] & \textbf{0.659} [0.645, 0.674] & 0.612 [0.591, 0.636] & & \\
Two effects, local $\sigma(b_p)$ & 0.643 [0.617, 0.670] & \textbf{0.659} [0.646, 0.674] & 0.612 [0.590, 0.636] & & \\
Free learner (propagated $\hat r_p$ as input) & 0.647 [0.622, 0.673] & \textbf{0.659} [0.645, 0.674] & 0.612 [0.591, 0.636] & & \\
Interaction-effect propagation & \textbf{0.655} [0.631, 0.682] & 0.658 [0.644, 0.673] & 0.612 [0.590, 0.636] & & \\
\midrule
\multicolumn{6}{l}{\emph{In-domain}} \\
PRR [95\% CI] & Sequential ($n{=}9$) & Fully conn. ($n{=}9$) & Hierarchy ($n{=}6$) & & \\
\midrule
PropUQ-MAS (training-free) & 0.161 [0.096, 0.223] & 0.144 [0.110, 0.180] & 0.030 [$-$0.030, 0.102] & & \\
Raw verbalized uncertainty & 0.097 [0.047, 0.148] & 0.087 [0.057, 0.117] & $-$0.006 [$-$0.061, 0.055] & & \\
Receiver Only & 0.109 [0.059, 0.159] & 0.088 [0.058, 0.119] & $-$0.004 [$-$0.062, 0.057] & & \\
Receiver-text & 0.227 [0.162, 0.296] & 0.254 [0.217, 0.286] & \textbf{0.212} [0.146, 0.272] & & \\
Interaction without parent state & 0.239 [0.177, 0.301] & 0.283 [0.248, 0.315] & 0.201 [0.136, 0.262] & & \\
Free learner, local $\sigma(b_p)$ & 0.242 [0.182, 0.303] & 0.284 [0.250, 0.317] & 0.179 [0.118, 0.241] & & \\
Two effects, local $\sigma(b_p)$ & 0.244 [0.180, 0.308] & \textbf{0.285} [0.250, 0.318] & 0.166 [0.104, 0.227] & & \\
Free learner (propagated $\hat r_p$ as input) & 0.245 [0.185, 0.306] & 0.284 [0.250, 0.317] & 0.179 [0.118, 0.241] & & \\
Interaction-effect propagation & \textbf{0.261} [0.198, 0.324] & 0.283 [0.249, 0.316] & 0.166 [0.104, 0.227] & & \\
\midrule
\multicolumn{6}{l}{\emph{Transfer}} \\
AUROC [95\% CI] & Sequential ($n{=}6$) & Fully conn. ($n{=}6$) & Hierarchy ($n{=}3$) & $\tau$ airline ($n{=}6$) & $\tau$ retail ($n{=}6$) \\
\midrule
PropUQ-MAS (training-free) & \textbf{0.576} [0.560, 0.593] & \textbf{0.577} [0.564, 0.590] & 0.506 [0.483, 0.529] & \textbf{0.586} [0.556, 0.616] & \textbf{0.712} [0.663, 0.755] \\
Raw verbalized uncertainty & 0.536 [0.524, 0.549] & 0.542 [0.530, 0.553] & 0.496 [0.476, 0.514] & 0.553 [0.523, 0.584] & 0.683 [0.633, 0.734] \\
Receiver Only & 0.537 [0.525, 0.550] & 0.542 [0.530, 0.552] & 0.497 [0.476, 0.516] & 0.464 [0.434, 0.492] & 0.490 [0.428, 0.550] \\
Receiver-text & 0.542 [0.522, 0.560] & 0.539 [0.525, 0.554] & 0.499 [0.474, 0.526] & 0.426 [0.393, 0.459] & 0.409 [0.345, 0.476] \\
Interaction without parent state & 0.548 [0.527, 0.565] & 0.552 [0.537, 0.567] & 0.519 [0.493, 0.544] & 0.500 [0.469, 0.534] & 0.537 [0.475, 0.600] \\
Free learner, local $\sigma(b_p)$ & 0.546 [0.525, 0.563] & 0.551 [0.536, 0.566] & 0.521 [0.496, 0.546] & -- & -- \\
Two effects, local $\sigma(b_p)$ & 0.552 [0.532, 0.569] & 0.554 [0.539, 0.569] & \textbf{0.524} [0.499, 0.550] & -- & -- \\
Free learner (propagated $\hat r_p$ as input) & 0.550 [0.529, 0.567] & 0.551 [0.536, 0.566] & 0.521 [0.496, 0.546] & -- & -- \\
Interaction-effect propagation & 0.569 [0.549, 0.587] & 0.555 [0.540, 0.570] & \textbf{0.524} [0.499, 0.550] & 0.521 [0.489, 0.554] & 0.564 [0.503, 0.623] \\
\midrule
\multicolumn{6}{l}{\emph{Transfer}} \\
PRR [95\% CI] & Sequential ($n{=}6$) & Fully conn. ($n{=}6$) & Hierarchy ($n{=}3$) & $\tau$ airline ($n{=}6$) & $\tau$ retail ($n{=}6$) \\
\midrule
PropUQ-MAS (training-free) & \textbf{0.172} [0.138, 0.207] & \textbf{0.169} [0.143, 0.195] & 0.023 [$-$0.055, 0.100] & \textbf{0.364} [0.278, 0.445] & \textbf{0.879} [0.789, 0.944] \\
Raw verbalized uncertainty & 0.091 [0.065, 0.118] & 0.091 [0.069, 0.112] & 0.001 [$-$0.066, 0.062] & 0.351 [0.266, 0.427] & 0.713 [0.598, 0.826] \\
Receiver Only & 0.090 [0.064, 0.118] & 0.091 [0.069, 0.113] & 0.006 [$-$0.061, 0.072] & $-$0.025 [$-$0.116, 0.062] & $-$0.132 [$-$0.323, 0.069] \\
Receiver-text & 0.089 [0.054, 0.124] & 0.072 [0.045, 0.099] & $-$0.012 [$-$0.098, 0.080] & $-$0.183 [$-$0.282, $-$0.084] & $-$0.434 [$-$0.704, $-$0.163] \\
Interaction without parent state & 0.097 [0.061, 0.131] & 0.116 [0.089, 0.143] & 0.046 [$-$0.031, 0.128] & 0.068 [$-$0.027, 0.168] & 0.060 [$-$0.171, 0.281] \\
Free learner, local $\sigma(b_p)$ & 0.098 [0.061, 0.131] & 0.114 [0.087, 0.141] & \textbf{0.052} [$-$0.021, 0.133] & -- & -- \\
Two effects, local $\sigma(b_p)$ & 0.107 [0.070, 0.141] & 0.120 [0.093, 0.148] & 0.038 [$-$0.037, 0.120] & -- & -- \\
Free learner (propagated $\hat r_p$ as input) & 0.105 [0.067, 0.136] & 0.113 [0.086, 0.141] & \textbf{0.052} [$-$0.021, 0.133] & -- & -- \\
Interaction-effect propagation & 0.139 [0.101, 0.173] & 0.120 [0.093, 0.147] & 0.038 [$-$0.037, 0.120] & 0.147 [0.052, 0.240] & 0.196 [$-$0.027, 0.398] \\
\bottomrule
\end{tabular}}
\caption{Group means with 95\% paired-bootstrap CIs (AUROC and PRR, in-domain and transfer). Bold: best mean in each column of each block.}
\label{tab:groupci}
\end{table*}


==> tables/incremental_full.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{llcc}
\toprule
Parent risks & Added to $b_{\mathrm{sink}}$ & $\Delta$NLL [CI] & $\Delta$AUROC [CI] \\
\midrule
\multicolumn{4}{l}{\emph{WebArena} (receiver evidence alone: NLL 0.440, AUROC 0.748)} \\
propagated $\hat r_p$ & parent risks & +0.064 [0.014, 0.124] & +0.105 [0.022, 0.184] \\
parent-local $\sigma(b_p)$ & parent risks & $-$0.005 [$-$0.026, 0.017] & +0.023 [$-$0.016, 0.058] \\
oracle & true parent states & +0.082 [0.027, 0.134] & +0.125 [0.043, 0.205] \\
\multicolumn{4}{l}{\emph{AppWorld} (receiver evidence alone: NLL 0.591, AUROC 0.630)} \\
propagated $\hat r_p$ & parent risks & +0.007 [$-$0.011, 0.025] & +0.023 [$-$0.020, 0.066] \\
parent-local $\sigma(b_p)$ & parent risks & +0.015 [$-$0.004, 0.033] & +0.032 [$-$0.010, 0.073] \\
oracle & true parent states & +0.241 [0.162, 0.321] & +0.278 [0.197, 0.356] \\
\bottomrule
\end{tabular}}
\caption{Incremental-information regressions: out-of-fold L2 logistic regression ($C{=}0.1$) of executor error on the receiver's local evidence plus role-aggregated (mean, and max where a role has several parents) parent features, on the same grouped folds; task-clustered 95\% CI. Results with $C{=}1$ are similar.}
\label{tab:incremental}
\end{table}


==> tables/interp_full.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{4}{c}{WebArena} & \multicolumn{4}{c}{AppWorld} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
 & \multicolumn{2}{c}{NP} & \multicolumn{2}{c}{PME} & \multicolumn{2}{c}{NP} & \multicolumn{2}{c}{PME} \\
$\varepsilon$ & NLL & AUROC & NLL & AUROC & NLL & AUROC & NLL & AUROC \\
\midrule
0 & 0.463 & 0.835 & 0.458 & 0.815 & 0.634 & 0.616 & 0.607 & 0.618 \\
0.25 & 0.389 & 0.876 & 0.402 & 0.867 & 0.581 & 0.702 & 0.562 & 0.710 \\
0.5 & 0.349 & 0.895 & 0.363 & 0.892 & 0.539 & 0.755 & 0.526 & 0.762 \\
0.75 & 0.333 & 0.896 & 0.339 & 0.897 & 0.508 & 0.786 & 0.500 & 0.789 \\
1 & 0.333 & 0.889 & 0.333 & 0.889 & 0.488 & 0.801 & 0.488 & 0.801 \\
\bottomrule
\end{tabular}}
\caption{Executor risk with the state-supervised potentials when parent risks are mixed with the true parent states, $r_p=(1-\varepsilon)\hat r_p+\varepsilon E_p$.}
\label{tab:interp}
\end{table}


==> tables/ladder.tex <==
\begin{table*}[t]
\centering\small
\setlength{\tabcolsep}{4.2pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{11}{l}{\emph{In-domain}} \\
 & \multicolumn{2}{c}{Sequential ($n{=}9$)} & \multicolumn{2}{c}{Fully conn. ($n{=}9$)} & \multicolumn{2}{c}{Hierarchy ($n{=}6$)} & & & & \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Estimator & AUROC & PRR & AUROC & PRR & AUROC & PRR & & & & \\
\midrule
PropUQ-MAS (training-free) & 0.584 & 0.161 & 0.582 & 0.144 & 0.529 & 0.030 & & & & \\
\midrule
Raw verbalized uncertainty & 0.543 & 0.097 & 0.545 & 0.087 & 0.502 & $-$0.006 & & & & \\
Receiver Only & 0.548 & 0.109 & 0.545 & 0.088 & 0.502 & $-$0.004 & & & & \\
Receiver-text & 0.636 & 0.227 & 0.640 & 0.254 & 0.616 & \textbf{0.212} & & & & \\
Interaction without parent state & 0.640 & 0.239 & 0.658 & 0.283 & \textbf{0.621} & 0.201 & & & & \\
Free learner, local $\sigma(b_p)$ & 0.641 & 0.242 & \textbf{0.659} & 0.284 & 0.612 & 0.179 & & & & \\
Two effects, local $\sigma(b_p)$ & 0.643 & 0.244 & \textbf{0.659} & \textbf{0.285} & 0.612 & 0.166 & & & & \\
Free learner (propagated $\hat r_p$ as input) & 0.647 & 0.245 & \textbf{0.659} & 0.284 & 0.612 & 0.179 & & & & \\
Interaction-effect propagation & \textbf{0.655} & \textbf{0.261} & 0.658 & 0.283 & 0.612 & 0.166 & & & & \\
\midrule
\multicolumn{11}{l}{\emph{Transfer}} \\
 & \multicolumn{2}{c}{Sequential ($n{=}6$)} & \multicolumn{2}{c}{Fully conn. ($n{=}6$)} & \multicolumn{2}{c}{Hierarchy ($n{=}3$)} & \multicolumn{2}{c}{$\tau$ airline ($n{=}6$)} & \multicolumn{2}{c}{$\tau$ retail ($n{=}6$)} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
Estimator & AUROC & PRR & AUROC & PRR & AUROC & PRR & AUROC & PRR & AUROC & PRR \\
\midrule
PropUQ-MAS (training-free) & \textbf{0.576} & \textbf{0.172} & \textbf{0.577} & \textbf{0.169} & 0.506 & 0.023 & \textbf{0.586} & \textbf{0.364} & \textbf{0.712} & \textbf{0.879} \\
\midrule
Raw verbalized uncertainty & 0.536 & 0.091 & 0.542 & 0.091 & 0.496 & 0.001 & 0.553 & 0.351 & 0.683 & 0.713 \\
Receiver Only & 0.537 & 0.090 & 0.542 & 0.091 & 0.497 & 0.006 & 0.464 & $-$0.025 & 0.490 & $-$0.132 \\
Receiver-text & 0.542 & 0.089 & 0.539 & 0.072 & 0.499 & $-$0.012 & 0.426 & $-$0.183 & 0.409 & $-$0.434 \\
Interaction without parent state & 0.548 & 0.097 & 0.552 & 0.116 & 0.519 & 0.046 & 0.500 & 0.068 & 0.537 & 0.060 \\
Free learner, local $\sigma(b_p)$ & 0.546 & 0.098 & 0.551 & 0.114 & 0.521 & \textbf{0.052} & -- & -- & -- & -- \\
Two effects, local $\sigma(b_p)$ & 0.552 & 0.107 & 0.554 & 0.120 & \textbf{0.524} & 0.038 & -- & -- & -- & -- \\
Free learner (propagated $\hat r_p$ as input) & 0.550 & 0.105 & 0.551 & 0.113 & 0.521 & \textbf{0.052} & -- & -- & -- & -- \\
Interaction-effect propagation & 0.569 & 0.139 & 0.555 & 0.120 & \textbf{0.524} & 0.038 & 0.521 & 0.147 & 0.564 & 0.196 \\
\bottomrule
\end{tabular}}
\caption{Final-node error-risk ranking of the controlled-QA estimators in every group. Upper block: in-domain; lower block: transfer, i.e.\ each system's estimators trained on MedQA and applied to its GSM8K and WebQA traces, and the sequential system's estimators applied to $\tau$-bench. Each row adds one source of information to the row above, except that the free learner and interaction-effect propagation receive the same information and differ only in how the propagated parent risk is used; the free learner and the local-risk variants were not run on $\tau$-bench (--). All rows except the raw uncertainty and PropUQ-MAS are separately trained (3 seeds, 5 question-level folds) with the same encoder, folds and optimizer. Values are means over the settings of a group (each setting weighted equally) of the seed mean. PRR is tie-aware with 50\% maximum rejection. 95\% bootstrap CIs for every entry are in Table~\ref{tab:groupci}; CIs for the step differences are in Table~\ref{tab:steps}. $\tau$-bench retail has error rates of 0.94--0.98 (8--20 correct items per setting). Bold: best value in each column of each block.}
\label{tab:ladder}
\end{table*}


==> tables/np_vs_pme.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{lcc}
\toprule
NLL(PME) $-$ NLL(NP), mean [CI] (frac.\ NP better) & WebArena & AppWorld \\
\midrule
shared recursive-soft potentials (trained with NP) & $-$0.0148 [$-$0.0355, $-$0.0014] (0.71) & $-$0.0000 [$-$0.0001, $-$0.0000] (0.63) \\
shared recursive-soft potentials (trained with PME) & $-$0.0138 [$-$0.0331, $-$0.0014] (0.71) & $-$0.0000 [$-$0.0001, $-$0.0000] (0.64) \\
shared state-supervised potentials & $-$0.0051 [$-$0.0561, 0.0440] (0.59) & $-$0.0270 [$-$0.0517, $-$0.0064] (0.69) \\
separately trained & $-$0.0095 [$-$0.0224, $-$0.0009] (0.60) & $-$0.0000 [$-$0.0000, $-$0.0000] (0.46) \\
\bottomrule
\end{tabular}}
\caption{NP versus PME inference on the executor (task-clustered 95\% CI; fraction of trajectories on which NP has lower NLL).}
\label{tab:npvspme}
\end{table}


==> tables/persetting.tex <==
\begin{table*}[p]
\centering\scriptsize
\setlength{\tabcolsep}{3.2pt}
\resizebox{\textwidth}{!}{\begin{tabular}{llllrrccccccccc}
\toprule
System & Data & Model & Train & $n$ & err. & PropUQ & Raw & RO & RT & Int. & Free-loc. & IE-loc. & Free & IE \\
\midrule
seq. & gsm8k & 0.6B & gsm8k & 239 & 0.32 & 0.622 & 0.551 & 0.546 & 0.646 & 0.660 & 0.661 & 0.665 & 0.658 & \textbf{0.667} \\
seq. & gsm8k & 0.6B & medqa & 239 & 0.32 & \textbf{0.622} & 0.551 & 0.549 & 0.551 & 0.527 & 0.527 & 0.536 & 0.526 & 0.539 \\
seq. & gsm8k & 1.7B & gsm8k & 1008 & 0.15 & 0.591 & 0.523 & 0.523 & 0.711 & 0.690 & 0.691 & 0.690 & 0.706 & \textbf{0.718} \\
seq. & gsm8k & 1.7B & medqa & 1008 & 0.15 & 0.591 & 0.523 & 0.523 & 0.543 & 0.564 & 0.560 & 0.566 & 0.568 & \textbf{0.613} \\
seq. & gsm8k & 4B & gsm8k & 1319 & 0.13 & 0.570 & 0.519 & 0.526 & 0.720 & 0.730 & 0.729 & 0.730 & 0.732 & \textbf{0.742} \\
seq. & gsm8k & 4B & medqa & 1319 & 0.13 & 0.570 & 0.519 & 0.527 & 0.547 & 0.587 & 0.586 & 0.593 & 0.592 & \textbf{0.629} \\
seq. & medqa & 0.6B & medqa & 42 & 0.62 & 0.500 & 0.507 & 0.508 & \textbf{0.571} & 0.549 & 0.549 & 0.561 & 0.546 & 0.569 \\
seq. & medqa & 1.7B & medqa & 297 & 0.50 & 0.590 & 0.566 & 0.582 & \textbf{0.642} & 0.627 & 0.627 & 0.627 & 0.629 & 0.635 \\
seq. & medqa & 4B & medqa & 299 & 0.33 & 0.711 & 0.601 & 0.624 & 0.681 & 0.726 & 0.726 & 0.729 & 0.755 & \textbf{0.761} \\
seq. & $\tau$-airline & 0.6B & gsm8k & 200 & 0.65 & \textbf{0.657} & 0.581 & 0.581 & 0.538 & 0.552 & -- & -- & -- & 0.544 \\
seq. & $\tau$-airline & 0.6B & medqa & 200 & 0.65 & \textbf{0.657} & 0.581 & 0.581 & 0.471 & 0.511 & -- & -- & -- & 0.489 \\
seq. & $\tau$-airline & 1.7B & gsm8k & 200 & 0.59 & \textbf{0.538} & 0.535 & 0.535 & 0.382 & 0.439 & -- & -- & -- & 0.474 \\
seq. & $\tau$-airline & 1.7B & medqa & 200 & 0.59 & 0.538 & 0.535 & 0.374 & 0.639 & 0.698 & -- & -- & -- & \textbf{0.708} \\
seq. & $\tau$-airline & 4B & gsm8k & 200 & 0.71 & \textbf{0.563} & 0.543 & 0.403 & 0.221 & 0.461 & -- & -- & -- & 0.479 \\
seq. & $\tau$-airline & 4B & medqa & 200 & 0.71 & \textbf{0.563} & 0.543 & 0.311 & 0.302 & 0.336 & -- & -- & -- & 0.432 \\
seq. & $\tau$-retail & 0.6B & gsm8k & 360 & 0.98 & 0.697 & 0.642 & 0.642 & 0.600 & 0.719 & -- & -- & -- & \textbf{0.734} \\
seq. & $\tau$-retail & 0.6B & medqa & 360 & 0.98 & \textbf{0.697} & 0.642 & 0.642 & 0.545 & 0.513 & -- & -- & -- & 0.514 \\
seq. & $\tau$-retail & 1.7B & gsm8k & 338 & 0.94 & \textbf{0.698} & 0.641 & 0.641 & 0.461 & 0.655 & -- & -- & -- & 0.672 \\
seq. & $\tau$-retail & 1.7B & medqa & 338 & 0.94 & \textbf{0.698} & 0.641 & 0.309 & 0.278 & 0.310 & -- & -- & -- & 0.320 \\
seq. & $\tau$-retail & 4B & gsm8k & 367 & 0.96 & 0.741 & \textbf{0.768} & 0.364 & 0.285 & 0.700 & -- & -- & -- & 0.705 \\
seq. & $\tau$-retail & 4B & medqa & 367 & 0.96 & 0.741 & \textbf{0.768} & 0.342 & 0.285 & 0.322 & -- & -- & -- & 0.436 \\
seq. & webqa & 0.6B & webqa & 1302 & 0.63 & 0.552 & 0.531 & 0.531 & 0.567 & 0.581 & 0.584 & 0.584 & \textbf{0.586} & \textbf{0.586} \\
seq. & webqa & 0.6B & medqa & 1302 & 0.63 & \textbf{0.552} & 0.531 & 0.531 & 0.518 & 0.521 & 0.514 & 0.523 & 0.513 & 0.523 \\
seq. & webqa & 1.7B & webqa & 2410 & 0.54 & 0.564 & 0.551 & 0.551 & 0.599 & 0.602 & 0.602 & 0.602 & 0.603 & \textbf{0.605} \\
seq. & webqa & 1.7B & medqa & 2410 & 0.54 & \textbf{0.564} & 0.551 & 0.551 & 0.547 & 0.547 & 0.546 & 0.547 & 0.547 & 0.553 \\
seq. & webqa & 4B & webqa & 2421 & 0.48 & 0.559 & 0.539 & 0.539 & 0.585 & 0.600 & 0.600 & 0.600 & 0.604 & \textbf{0.610} \\
seq. & webqa & 4B & medqa & 2421 & 0.48 & \textbf{0.559} & 0.539 & 0.540 & 0.543 & 0.541 & 0.542 & 0.544 & 0.551 & \textbf{0.559} \\
\midrule
FC & gsm8k & 0.6B & gsm8k & 1157 & 0.28 & 0.571 & 0.538 & 0.537 & 0.689 & \textbf{0.720} & \textbf{0.720} & \textbf{0.720} & \textbf{0.720} & 0.719 \\
FC & gsm8k & 0.6B & medqa & 1157 & 0.28 & \textbf{0.571} & 0.538 & 0.537 & 0.509 & 0.503 & 0.504 & 0.506 & 0.505 & 0.512 \\
FC & gsm8k & 1.7B & gsm8k & 1314 & 0.26 & 0.544 & 0.520 & 0.520 & 0.697 & \textbf{0.712} & \textbf{0.712} & 0.711 & \textbf{0.712} & \textbf{0.712} \\
FC & gsm8k & 1.7B & medqa & 1314 & 0.26 & 0.544 & 0.520 & 0.520 & 0.549 & 0.549 & 0.544 & 0.548 & 0.544 & \textbf{0.552} \\
FC & gsm8k & 4B & gsm8k & 1315 & 0.09 & 0.649 & 0.586 & 0.584 & 0.713 & 0.757 & \textbf{0.758} & 0.756 & \textbf{0.758} & 0.756 \\
FC & gsm8k & 4B & medqa & 1315 & 0.09 & \textbf{0.649} & 0.586 & 0.585 & 0.591 & 0.628 & 0.627 & 0.632 & 0.626 & 0.627 \\
FC & medqa & 0.6B & medqa & 290 & 0.64 & 0.474 & 0.482 & 0.483 & \textbf{0.511} & 0.487 & 0.489 & 0.490 & 0.489 & 0.489 \\
FC & medqa & 1.7B & medqa & 300 & 0.50 & 0.582 & 0.560 & 0.558 & \textbf{0.673} & 0.650 & 0.654 & 0.652 & 0.654 & 0.649 \\
FC & medqa & 4B & medqa & 300 & 0.30 & 0.717 & 0.612 & 0.614 & 0.692 & 0.764 & 0.763 & \textbf{0.769} & 0.765 & 0.766 \\
FC & webqa & 0.6B & webqa & 2420 & 0.62 & 0.544 & 0.528 & 0.530 & 0.585 & \textbf{0.588} & \textbf{0.588} & 0.587 & \textbf{0.588} & 0.586 \\
FC & webqa & 0.6B & medqa & 2420 & 0.62 & \textbf{0.544} & 0.528 & 0.528 & 0.509 & 0.506 & 0.506 & 0.508 & 0.507 & 0.509 \\
FC & webqa & 1.7B & webqa & 2427 & 0.53 & 0.588 & 0.531 & 0.531 & 0.602 & 0.629 & 0.629 & \textbf{0.631} & 0.629 & 0.629 \\
FC & webqa & 1.7B & medqa & 2427 & 0.53 & \textbf{0.588} & 0.531 & 0.531 & 0.535 & 0.557 & 0.555 & 0.559 & 0.554 & 0.560 \\
FC & webqa & 4B & webqa & 2452 & 0.47 & 0.568 & 0.549 & 0.550 & 0.601 & 0.618 & 0.618 & 0.618 & 0.618 & \textbf{0.621} \\
FC & webqa & 4B & medqa & 2452 & 0.47 & 0.568 & 0.549 & 0.548 & 0.543 & 0.568 & 0.569 & \textbf{0.570} & 0.569 & 0.568 \\
\midrule
hier. & gsm8k & 0.6B & gsm8k & 981 & 0.74 & 0.513 & 0.501 & 0.501 & \textbf{0.554} & 0.550 & 0.553 & 0.552 & 0.553 & 0.552 \\
hier. & gsm8k & 0.6B & medqa & 981 & 0.74 & \textbf{0.513} & 0.501 & 0.501 & 0.508 & 0.491 & 0.507 & 0.504 & 0.507 & 0.504 \\
hier. & gsm8k & 1.7B & gsm8k & 1317 & 0.92 & 0.485 & 0.495 & 0.499 & \textbf{0.547} & 0.531 & 0.528 & 0.531 & 0.528 & 0.531 \\
hier. & gsm8k & 1.7B & medqa & 1317 & 0.92 & 0.485 & 0.495 & \textbf{0.499} & 0.452 & 0.495 & 0.491 & 0.491 & 0.491 & 0.491 \\
hier. & gsm8k & 4B & gsm8k & 1317 & 0.18 & 0.520 & 0.491 & 0.490 & \textbf{0.840} & 0.812 & 0.810 & 0.811 & 0.810 & 0.811 \\
hier. & gsm8k & 4B & medqa & 1317 & 0.18 & 0.520 & 0.491 & 0.490 & 0.537 & 0.572 & 0.565 & \textbf{0.577} & 0.565 & \textbf{0.577} \\
hier. & medqa & 0.6B & medqa & 230 & 0.64 & 0.398 & 0.414 & 0.409 & 0.556 & \textbf{0.557} & 0.510 & 0.497 & 0.510 & 0.497 \\
hier. & medqa & 1.7B & medqa & 299 & 0.52 & \textbf{0.565} & 0.504 & 0.504 & 0.551 & 0.559 & 0.558 & 0.563 & 0.558 & 0.563 \\
hier. & medqa & 4B & medqa & 299 & 0.31 & 0.695 & 0.608 & 0.608 & 0.649 & 0.715 & 0.715 & \textbf{0.717} & 0.715 & \textbf{0.717} \\
\bottomrule
\end{tabular}}
\caption{Per-setting final-node AUROC (seed means). Seq.: sequential; FC: fully connected; Raw: raw verbalized uncertainty; RO: Receiver Only; RT: Receiver-text; Int.: interaction without parent state; Free: free learner (not run on $\tau$-bench); -loc.: with the parent's local risk; IE: interaction-effect propagation. err.: final-node error rate on the paired test items. Bold: best estimator in each setting.}
\label{tab:persetting}
\end{table*}


==> tables/prr_steps.tex <==
\begin{table*}[t]
\centering\small
\setlength{\tabcolsep}{3.5pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{l}{\emph{In-domain}} \\
Step ($\Delta$PRR) & Sequential ($n{=}9$) & Fully conn. ($n{=}9$) & Hierarchy ($n{=}6$) & & \\
\midrule
Receiver Only vs.\ raw uncertainty & \makecell{+0.012\\{\scriptsize[$-$0.004, +0.029]\;4/9}} & \makecell{+0.001\\{\scriptsize[$-$0.002, +0.004]\;6/9}} & \makecell{+0.002\\{\scriptsize[$-$0.007, +0.008]\;3/6}} & & \\
Receiver-text vs.\ Receiver Only & \makecell{+0.118$^\ast$\\{\scriptsize[+0.054, +0.177]\;8/9}} & \makecell{+0.165$^\ast$\\{\scriptsize[+0.130, +0.200]\;9/9}} & \makecell{+0.216$^\ast$\\{\scriptsize[+0.148, +0.282]\;6/6}} & & \\
Interaction vs.\ Receiver-text & \makecell{+0.012\\{\scriptsize[$-$0.020, +0.042]\;6/9}} & \makecell{+0.029$^\ast$\\{\scriptsize[+0.010, +0.048]\;7/9}} & \makecell{$-$0.011\\{\scriptsize[$-$0.045, +0.026]\;2/6}} & & \\
IE propagation vs.\ free learner & \makecell{+0.016\\{\scriptsize[$-$0.000, +0.035]\;7/9}} & \makecell{$-$0.001\\{\scriptsize[$-$0.005, +0.003]\;3/9}} & \makecell{$-$0.013\\{\scriptsize[$-$0.035, +0.010]\;5/6}} & & \\
IE propagation vs.\ local parent risk & \makecell{+0.017$^\ast$\\{\scriptsize[+0.002, +0.033]\;8/9}} & \makecell{$-$0.002\\{\scriptsize[$-$0.005, +0.001]\;2/9}} & \makecell{+0.000\\{\scriptsize[+0.000, +0.000]\;0/6}} & & \\
Free learner vs.\ local parent risk & \makecell{+0.003\\{\scriptsize[$-$0.004, +0.011]\;6/9}} & \makecell{+0.000\\{\scriptsize[$-$0.001, +0.001]\;3/9}} & \makecell{+0.000\\{\scriptsize[+0.000, +0.000]\;0/6}} & & \\
\midrule
IE propagation vs.\ Receiver-text & \makecell{+0.034$^\ast$\\{\scriptsize[+0.003, +0.066]\;7/9}} & \makecell{+0.029$^\ast$\\{\scriptsize[+0.010, +0.049]\;7/9}} & \makecell{$-$0.045$^\ast$\\{\scriptsize[$-$0.083, $-$0.008]\;1/6}} & & \\
IE propagation vs.\ PropUQ-MAS & \makecell{+0.100$^\ast$\\{\scriptsize[+0.039, +0.165]\;9/9}} & \makecell{+0.139$^\ast$\\{\scriptsize[+0.100, +0.176]\;9/9}} & \makecell{+0.136$^\ast$\\{\scriptsize[+0.074, +0.201]\;5/6}} & & \\
\midrule
\multicolumn{6}{l}{\emph{Transfer}} \\
Step ($\Delta$PRR) & Sequential ($n{=}6$) & Fully conn. ($n{=}6$) & Hierarchy ($n{=}3$) & $\tau$ airline ($n{=}6$) & $\tau$ retail ($n{=}6$) \\
\midrule
Receiver Only vs.\ raw uncertainty & \makecell{$-$0.001\\{\scriptsize[$-$0.003, +0.001]\;3/6}} & \makecell{+0.000\\{\scriptsize[$-$0.002, +0.003]\;4/6}} & \makecell{+0.006\\{\scriptsize[$-$0.009, +0.017]\;1/3}} & \makecell{$-$0.376$^\ast$\\{\scriptsize[$-$0.481, $-$0.279]\;2/6}} & \makecell{$-$0.846$^\ast$\\{\scriptsize[$-$1.045, $-$0.637]\;0/6}} \\
Receiver-text vs.\ Receiver Only & \makecell{$-$0.001\\{\scriptsize[$-$0.034, +0.033]\;3/6}} & \makecell{$-$0.019\\{\scriptsize[$-$0.043, +0.006]\;2/6}} & \makecell{$-$0.018\\{\scriptsize[$-$0.096, +0.070]\;2/3}} & \makecell{$-$0.157$^\ast$\\{\scriptsize[$-$0.260, $-$0.040]\;2/6}} & \makecell{$-$0.302$^\ast$\\{\scriptsize[$-$0.573, $-$0.037]\;1/6}} \\
Interaction vs.\ Receiver-text & \makecell{+0.008\\{\scriptsize[$-$0.013, +0.029]\;3/6}} & \makecell{+0.044$^\ast$\\{\scriptsize[+0.025, +0.063]\;5/6}} & \makecell{+0.058\\{\scriptsize[$-$0.006, +0.119]\;2/3}} & \makecell{+0.251$^\ast$\\{\scriptsize[+0.163, +0.336]\;6/6}} & \makecell{+0.494$^\ast$\\{\scriptsize[+0.279, +0.709]\;5/6}} \\
IE propagation vs.\ free learner & \makecell{+0.035$^\ast$\\{\scriptsize[+0.021, +0.048]\;6/6}} & \makecell{+0.006$^\ast$\\{\scriptsize[+0.003, +0.010]\;4/6}} & \makecell{$-$0.014\\{\scriptsize[$-$0.046, +0.016]\;1/3}} & -- & -- \\
IE propagation vs.\ local parent risk & \makecell{+0.032$^\ast$\\{\scriptsize[+0.021, +0.044]\;5/6}} & \makecell{$-$0.001\\{\scriptsize[$-$0.005, +0.004]\;4/6}} & \makecell{+0.000\\{\scriptsize[+0.000, +0.000]\;1/3}} & -- & -- \\
Free learner vs.\ local parent risk & \makecell{+0.007$^\ast$\\{\scriptsize[+0.002, +0.012]\;3/6}} & \makecell{$-$0.000\\{\scriptsize[$-$0.001, +0.000]\;2/6}} & \makecell{+0.000\\{\scriptsize[+0.000, +0.000]\;0/3}} & -- & -- \\
\midrule
IE propagation vs.\ Receiver-text & \makecell{+0.050$^\ast$\\{\scriptsize[+0.027, +0.073]\;5/6}} & \makecell{+0.048$^\ast$\\{\scriptsize[+0.028, +0.067]\;5/6}} & \makecell{+0.049\\{\scriptsize[$-$0.011, +0.111]\;2/3}} & \makecell{+0.330$^\ast$\\{\scriptsize[+0.232, +0.422]\;6/6}} & \makecell{+0.630$^\ast$\\{\scriptsize[+0.411, +0.838]\;5/6}} \\
IE propagation vs.\ PropUQ-MAS & \makecell{$-$0.033\\{\scriptsize[$-$0.071, +0.003]\;2/6}} & \makecell{$-$0.049$^\ast$\\{\scriptsize[$-$0.074, $-$0.024]\;2/6}} & \makecell{+0.015\\{\scriptsize[$-$0.077, +0.120]\;2/3}} & \makecell{$-$0.217$^\ast$\\{\scriptsize[$-$0.315, $-$0.110]\;1/6}} & \makecell{$-$0.684$^\ast$\\{\scriptsize[$-$0.897, $-$0.470]\;1/6}} \\
\bottomrule
\end{tabular}}
\caption{As Table~\ref{tab:steps}, for PRR.}
\label{tab:prrsteps}
\end{table*}


==> tables/qa_branch.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{In-domain} & \multicolumn{3}{c}{Transfer} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
 & Seq. & FC & Hier. & Seq. & FC & Hier. \\
\midrule
Parent-risk AUROC & 0.672 & 0.642 & 0.568 & 0.544 & 0.544 & 0.549 \\
Parent-risk std.\ dev. & 0.117 & 0.093 & 0.021 & 0.067 & 0.079 & 0.018 \\
\midrule Median $|\Delta_{pv}|$ & 1.53 & 0.54 & 0.13 & 2.67 & 0.52 & 0.31 \\
Edges with $|\Delta_{pv}|{<}0.1$ & 0.07 & 0.08 & 0.68 & 0.21 & 0.28 & 0.65 \\
Edges with $\Delta_{pv}{>}0$ & 0.89 & 0.17 & 0.34 & 0.75 & 0.49 & 0.46 \\
\bottomrule
\end{tabular}}
\caption{Parent risk and branch separation $\Delta_{pv}=\delta^{(1)}_{pv}-\delta^{(0)}_{pv}$ on the final node's incoming edges, for interaction-effect propagation trained end to end (\S\ref{sec:learning}). Parent-risk AUROC: how well the propagated parent risk ranks true parent errors; std.\ dev.: its spread across items; $\Delta_{pv}{>}0$: share of edges on which the effect for a wrong sender exceeds that for a correct one. Seq.: sequential; FC: fully connected. Values average settings.}
\label{tab:qabranch}
\end{table}


==> tables/qa_gsm8k.tex <==
\begin{table*}[tp]
\centering\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{Sequential} & \multicolumn{3}{c}{Fully connected} & \multicolumn{3}{c}{Hierarchy} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Estimator & NLL & Brier & AUROC & NLL & Brier & AUROC & NLL & Brier & AUROC \\
\midrule
\multicolumn{10}{l}{\emph{In-domain}: verbalized $u$} \\
Receiver-Only & 0.377 & 0.112 & 0.557 & 0.352 & 0.101 & 0.572 & 0.345 & 0.100 & 0.612 \\
Receiver-Text & 0.373 & 0.112 & 0.654 & 0.341 & 0.099 & 0.688 & 0.332 & \textbf{0.096} & 0.749 \\
Free Learner & 0.363 & 0.109 & 0.700 & 0.320 & \textbf{0.094} & \textbf{0.759} & 0.338 & 0.098 & \textbf{0.778} \\
Interaction-Effect Propagation & \textbf{0.362} & \textbf{0.108} & \textbf{0.701} & \textbf{0.318} & \textbf{0.094} & 0.757 & \textbf{0.329} & \textbf{0.096} & \textbf{0.778} \\
\cmidrule(lr){1-10}
PropUQ-MAS & 2.354 & 0.193 & 0.605 & 1.231 & 0.150 & 0.678 & 0.807 & 0.129 & 0.648 \\
\midrule
\multicolumn{10}{l}{\emph{In-domain}: MSP $u$} \\
Receiver-Only & 0.380 & 0.115 & 0.602 & 0.351 & 0.101 & 0.534 & 0.344 & 0.099 & 0.651 \\
Receiver-Text & 0.374 & 0.112 & 0.645 & 0.343 & 0.100 & 0.666 & 0.339 & 0.098 & 0.723 \\
Free Learner & \textbf{0.370} & \textbf{0.111} & 0.655 & 0.319 & \textbf{0.094} & 0.758 & 0.316 & 0.094 & \textbf{0.810} \\
Interaction-Effect Propagation & 0.372 & 0.112 & \textbf{0.666} & \textbf{0.318} & \textbf{0.094} & \textbf{0.763} & \textbf{0.309} & \textbf{0.092} & 0.808 \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.462 & 0.141 & 0.544 & 0.366 & 0.104 & 0.652 & 0.322 & 0.093 & 0.743 \\
\midrule
\multicolumn{10}{l}{\emph{In-domain}: entropy $u$} \\
Receiver-Only & 0.379 & 0.114 & 0.626 & 0.349 & 0.101 & 0.516 & 0.340 & 0.098 & 0.654 \\
Receiver-Text & 0.370 & 0.111 & 0.667 & 0.343 & 0.100 & 0.667 & 0.340 & 0.098 & 0.728 \\
Free Learner & \textbf{0.367} & \textbf{0.110} & 0.656 & 0.307 & 0.091 & 0.775 & \textbf{0.294} & \textbf{0.088} & \textbf{0.833} \\
Interaction-Effect Propagation & 0.371 & 0.112 & \textbf{0.668} & \textbf{0.303} & \textbf{0.089} & \textbf{0.778} & 0.296 & \textbf{0.088} & 0.830 \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.414 & 0.122 & 0.564 & 0.357 & 0.102 & 0.681 & 0.323 & 0.095 & 0.764 \\
\midrule
\multicolumn{10}{l}{\emph{Transfer from MedQA}: verbalized $u$} \\
Receiver-Only & 0.701 & 0.253 & 0.557 & 0.634 & 0.224 & 0.571 & 0.616 & 0.215 & 0.612 \\
Receiver-Text & 0.633 & 0.223 & 0.540 & 0.590 & 0.204 & 0.573 & 0.584 & 0.201 & 0.578 \\
Free Learner & \textbf{0.574} & 0.195 & 0.573 & 0.546 & 0.187 & 0.658 & 0.461 & 0.145 & 0.625 \\
Interaction-Effect Propagation & 0.593 & 0.204 & 0.567 & \textbf{0.524} & 0.178 & 0.655 & \textbf{0.458} & 0.144 & 0.626 \\
\cmidrule(lr){1-10}
PropUQ-MAS & 2.354 & \textbf{0.193} & \textbf{0.605} & 1.231 & \textbf{0.150} & \textbf{0.678} & 0.807 & \textbf{0.129} & \textbf{0.648} \\
\midrule
\multicolumn{10}{l}{\emph{Transfer from MedQA}: MSP $u$} \\
Receiver-Only & 0.712 & 0.259 & \textbf{0.602} & 0.638 & 0.226 & 0.572 & 0.633 & 0.223 & 0.621 \\
Receiver-Text & 0.616 & 0.220 & 0.568 & 0.552 & 0.189 & 0.528 & 0.584 & 0.204 & 0.563 \\
Free Learner & 0.545 & 0.188 & 0.579 & 0.473 & 0.160 & 0.597 & 0.434 & 0.145 & 0.655 \\
Interaction-Effect Propagation & 0.580 & 0.204 & 0.581 & 0.473 & 0.161 & 0.613 & 0.441 & 0.149 & 0.659 \\
\cmidrule(lr){1-10}
PropUQ-MAS & \textbf{0.462} & \textbf{0.141} & 0.544 & \textbf{0.366} & \textbf{0.104} & \textbf{0.652} & \textbf{0.322} & \textbf{0.093} & \textbf{0.743} \\
\midrule
\multicolumn{10}{l}{\emph{Transfer from MedQA}: entropy $u$} \\
Receiver-Only & 0.722 & 0.263 & \textbf{0.626} & 0.637 & 0.225 & 0.589 & 0.634 & 0.223 & 0.672 \\
Receiver-Text & 0.597 & 0.211 & 0.581 & 0.538 & 0.184 & 0.539 & 0.561 & 0.195 & 0.567 \\
Free Learner & 0.544 & 0.188 & 0.583 & 0.460 & 0.155 & 0.620 & 0.448 & 0.150 & 0.650 \\
Interaction-Effect Propagation & 0.549 & 0.191 & 0.594 & 0.468 & 0.160 & 0.627 & 0.448 & 0.150 & 0.648 \\
\cmidrule(lr){1-10}
PropUQ-MAS & \textbf{0.414} & \textbf{0.122} & 0.564 & \textbf{0.357} & \textbf{0.102} & \textbf{0.681} & \textbf{0.323} & \textbf{0.095} & \textbf{0.764} \\
\bottomrule
\end{tabular}}
\caption{Final-node error risk on GSM8K in the three controlled systems: means over the three Qwen3 model sizes of the seed mean (3 seeds, 5 question-level folds; 1{,}319 test questions, at most 8 per setting dropped for an incomplete trace or missing $u$). Blocks differ in the node uncertainty $u_v$ that every estimator receives: verbalized ($1-{}$self-reported probability of being correct), MSP ($1-{}$geometric-mean probability of the visible tokens) or entropy (mean top-20 token entropy over the visible tokens, divided by $\ln 20$). Learned rows share the encoder, folds and optimizer; Receiver-Text adds the receiver's own output to Receiver-Only, and Free Learner and Interaction-Effect Propagation read the same inputs and differ only in how they use the propagated parent risk. NLL uses risks clipped to $[10^{-6}, 1-10^{-6}]$; under verbalized $u$, 37--81\% of PropUQ-MAS outputs are exactly 0 or 1, so its NLL there depends on this clip. Transfer: estimators trained on MedQA traces of the same system and model; PropUQ-MAS is training-free, so its transfer rows repeat the in-domain ones. Bold: best value in each column of each block.}
\label{tab:qa-gsm8k}
\end{table*}


==> tables/qa_ladder_main.tex <==
\begin{table*}[t]
\centering\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{Sequential} & \multicolumn{3}{c}{Fully connected} & \multicolumn{3}{c}{Hierarchy} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Estimator & NLL & Brier & AUROC & NLL & Brier & AUROC & NLL & Brier & AUROC \\
\midrule
\multicolumn{10}{l}{\emph{In-domain} (9 / 9 / 6 settings)} \\
Receiver Only & 0.603 & 0.209 & 0.548 & 0.604 & 0.209 & 0.545 & 0.684 & 0.244 & 0.502 \\
Receiver-text & 0.590 & 0.204 & 0.636 & 0.584 & 0.201 & 0.640 & \textbf{0.660} & \textbf{0.237} & \textbf{0.616} \\
Free learner (propagated $\hat r_p$ as input) & 0.584 & \textbf{0.201} & 0.647 & 0.577 & 0.199 & \textbf{0.659} & 0.669 & 0.241 & 0.612 \\
Interaction-effect propagation & \textbf{0.582} & \textbf{0.201} & \textbf{0.655} & \textbf{0.575} & \textbf{0.198} & 0.658 & 0.666 & 0.239 & 0.612 \\
\cmidrule(lr){1-10}
PropUQ-MAS (training-free) & -- & -- & 0.584 & -- & -- & 0.582 & -- & -- & 0.529 \\
\midrule
\multicolumn{10}{l}{\emph{Transfer from MedQA to GSM8K and WebQA} (6 / 6 / 3 settings)} \\
Receiver Only & 0.663 & 0.236 & 0.537 & 0.675 & 0.241 & 0.542 & \textbf{0.577} & \textbf{0.195} & 0.497 \\
Receiver-text & \textbf{0.654} & 0.230 & 0.542 & \textbf{0.654} & \textbf{0.229} & 0.539 & 0.623 & 0.217 & 0.499 \\
Free learner (propagated $\hat r_p$ as input) & 0.664 & \textbf{0.229} & 0.550 & 0.718 & 0.236 & 0.551 & 0.778 & 0.261 & 0.521 \\
Interaction-effect propagation & 0.672 & 0.233 & 0.569 & 0.734 & 0.236 & 0.555 & 0.791 & 0.262 & \textbf{0.524} \\
\cmidrule(lr){1-10}
PropUQ-MAS (training-free) & -- & -- & \textbf{0.576} & -- & -- & \textbf{0.577} & -- & -- & 0.506 \\
\bottomrule
\end{tabular}}
\caption{Final-node error risk in the three controlled systems (means over settings of the seed mean; 3 seeds, 5 question-level folds). Learned rows share the encoder, folds and optimizer; Receiver-text adds the receiver's own output to Receiver Only, and the free learner and interaction-effect propagation read the same inputs and differ only in how they use the propagated parent risk. Transfer: estimators trained on MedQA traces of a system and applied to its GSM8K and WebQA traces. Bold: best value in each column of each block.}
\label{tab:qa}
\end{table*}


==> tables/qa_medqa.tex <==
\begin{table*}[t]
\centering\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{Sequential} & \multicolumn{3}{c}{Fully connected} & \multicolumn{3}{c}{Hierarchy} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Estimator & NLL & Brier & AUROC & NLL & Brier & AUROC & NLL & Brier & AUROC \\
\midrule
\multicolumn{10}{l}{\emph{In-domain}: verbalized $u$} \\
Receiver-Only & 0.668 & 0.237 & 0.514 & 0.654 & 0.231 & 0.531 & 0.643 & 0.226 & 0.587 \\
Receiver-Text & 0.662 & 0.235 & 0.568 & 0.649 & 0.228 & 0.551 & 0.630 & 0.220 & 0.608 \\
Free Learner & \textbf{0.651} & \textbf{0.229} & 0.604 & 0.647 & 0.227 & \textbf{0.598} & 0.625 & \textbf{0.218} & \textbf{0.622} \\
Interaction-Effect Propagation & \textbf{0.651} & \textbf{0.229} & \textbf{0.608} & \textbf{0.643} & \textbf{0.226} & \textbf{0.598} & \textbf{0.624} & \textbf{0.218} & \textbf{0.622} \\
\cmidrule(lr){1-10}
PropUQ-MAS & 3.776 & 0.374 & 0.576 & 2.454 & 0.322 & 0.582 & 1.938 & 0.299 & 0.583 \\
\midrule
\multicolumn{10}{l}{\emph{In-domain}: MSP $u$} \\
Receiver-Only & 0.669 & 0.238 & 0.560 & 0.655 & 0.231 & 0.511 & 0.647 & 0.228 & 0.597 \\
Receiver-Text & 0.653 & 0.231 & 0.602 & 0.652 & 0.230 & 0.547 & 0.637 & 0.224 & 0.590 \\
Free Learner & \textbf{0.646} & \textbf{0.227} & 0.613 & 0.637 & \textbf{0.223} & 0.597 & \textbf{0.601} & \textbf{0.209} & \textbf{0.655} \\
Interaction-Effect Propagation & \textbf{0.646} & 0.228 & \textbf{0.615} & \textbf{0.636} & \textbf{0.223} & 0.598 & \textbf{0.601} & \textbf{0.209} & 0.654 \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.748 & 0.260 & 0.564 & 0.864 & 0.306 & \textbf{0.602} & 0.951 & 0.291 & 0.617 \\
\midrule
\multicolumn{10}{l}{\emph{In-domain}: entropy $u$} \\
Receiver-Only & 0.672 & 0.239 & 0.562 & 0.655 & 0.231 & 0.526 & 0.648 & 0.228 & 0.612 \\
Receiver-Text & 0.650 & 0.229 & 0.597 & 0.652 & 0.229 & 0.554 & 0.629 & 0.220 & 0.607 \\
Free Learner & 0.645 & 0.227 & 0.612 & \textbf{0.627} & \textbf{0.219} & 0.615 & \textbf{0.597} & \textbf{0.207} & \textbf{0.669} \\
Interaction-Effect Propagation & \textbf{0.641} & \textbf{0.225} & \textbf{0.615} & \textbf{0.627} & \textbf{0.219} & 0.616 & \textbf{0.597} & \textbf{0.207} & \textbf{0.669} \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.813 & 0.287 & 0.572 & 1.017 & 0.350 & \textbf{0.635} & 1.084 & 0.343 & 0.613 \\
\bottomrule
\end{tabular}}
\caption{Final-node error risk on MedQA in the three controlled systems: means over the three Qwen3 model sizes of the seed mean (3 seeds, 5 question-level folds; 300 test questions, at most 1 per setting dropped for an incomplete trace or missing $u$). Protocols, estimators and layout as in Table~\ref{tab:qa-gsm8k}. MedQA is the transfer source, so there is no transfer block. Bold: best value in each column of each block.}
\label{tab:qa-medqa}
\end{table*}


==> tables/qa_prob_full.tex <==
\begin{table*}[t]
\centering\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{11}{l}{\emph{In-domain}} \\
 & \multicolumn{2}{c}{Sequential ($n{=}9$)} & \multicolumn{2}{c}{Fully conn. ($n{=}9$)} & \multicolumn{2}{c}{Hierarchy ($n{=}6$)} & & & & \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Estimator & NLL & Brier & NLL & Brier & NLL & Brier & & & & \\
\midrule
Raw verbalized uncertainty & 1.480 & 0.360 & 1.602 & 0.370 & 2.083 & 0.485 & & & & \\
Receiver Only & 0.603 & 0.209 & 0.604 & 0.209 & 0.684 & 0.244 & & & & \\
Receiver-text & 0.590 & 0.204 & 0.584 & 0.201 & \textbf{0.660} & \textbf{0.237} & & & & \\
Interaction without parent state & 0.588 & 0.203 & 0.578 & 0.199 & 0.666 & 0.239 & & & & \\
Free learner, local risk & 0.587 & 0.203 & 0.577 & 0.199 & 0.669 & 0.241 & & & & \\
Two effects, local risk & 0.588 & 0.203 & 0.576 & \textbf{0.198} & 0.666 & 0.239 & & & & \\
Free learner & 0.584 & \textbf{0.201} & 0.577 & 0.199 & 0.669 & 0.241 & & & & \\
Interaction-effect propagation & \textbf{0.582} & \textbf{0.201} & \textbf{0.575} & \textbf{0.198} & 0.666 & 0.239 & & & & \\
\midrule
\multicolumn{11}{l}{\emph{Transfer}} \\
 & \multicolumn{2}{c}{Sequential ($n{=}6$)} & \multicolumn{2}{c}{Fully conn. ($n{=}6$)} & \multicolumn{2}{c}{Hierarchy ($n{=}3$)} & \multicolumn{2}{c}{$\tau$ airline ($n{=}6$)} & \multicolumn{2}{c}{$\tau$ retail ($n{=}6$)} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
Estimator & NLL & Brier & NLL & Brier & NLL & Brier & NLL & Brier & NLL & Brier \\
\midrule
Raw verbalized uncertainty & 1.446 & 0.344 & 1.509 & 0.346 & 2.523 & 0.560 & 1.177 & 0.358 & \textbf{0.342} & \textbf{0.092} \\
Receiver Only & 0.663 & 0.236 & 0.675 & 0.241 & \textbf{0.577} & \textbf{0.195} & 0.897 & 0.324 & 0.903 & 0.323 \\
Receiver-text & \textbf{0.654} & 0.230 & \textbf{0.654} & \textbf{0.229} & 0.623 & 0.217 & \textbf{0.822} & \textbf{0.305} & 0.868 & 0.325 \\
Interaction without parent state & 0.667 & 0.231 & 0.711 & 0.234 & 0.761 & 0.263 & 0.878 & 0.317 & 0.703 & 0.242 \\
Free learner, local risk & 0.668 & 0.231 & 0.714 & 0.235 & 0.778 & 0.261 & -- & -- & -- & -- \\
Two effects, local risk & 0.667 & 0.232 & 0.707 & 0.234 & 0.791 & 0.262 & -- & -- & -- & -- \\
Free learner & 0.664 & \textbf{0.229} & 0.718 & 0.236 & 0.778 & 0.261 & -- & -- & -- & -- \\
Interaction-effect propagation & 0.672 & 0.233 & 0.734 & 0.236 & 0.791 & 0.262 & 0.896 & 0.313 & 0.546 & 0.181 \\
\bottomrule
\end{tabular}}
\caption{Probabilistic metrics of the QA estimators in every group (final node; means over settings of seed means). AUROC and PRR for the same cells are in Table~\ref{tab:ladder}. Bold: lowest value in each column of each block.}
\label{tab:qaprob}
\end{table*}


==> tables/qa_recursion.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{In-domain ($n{=}9$)} & \multicolumn{3}{c}{Transfer ($n{=}6$)} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Edge model & local & propag. & $\Delta$ & local & propag. & $\Delta$ \\
\midrule
\multicolumn{7}{l}{\emph{Sequential}} \\
Two state-cond.\ effects & \cellcolor{tabred}0.643 & \cellcolor{tabgreen}0.655 & \cellcolor{tabgreen}\makecell{+0.012$^\ast$\\{\scriptsize[0.006, 0.019]\;3/9}} & \cellcolor{tabred}0.552 & \cellcolor{tabgreen}0.569 & \cellcolor{tabgreen}\makecell{+0.018$^\ast$\\{\scriptsize[0.013, 0.023]\;3/6}} \\
Free learner & \cellcolor{tabred}0.641 & \cellcolor{tabgreen}0.647 & \cellcolor{tabgreen}\makecell{+0.006$^\ast$\\{\scriptsize[0.002, 0.009]\;2/9}} & \cellcolor{tabred}0.546 & \cellcolor{tabgreen}0.550 & \cellcolor{tabgreen}\makecell{+0.004$^\ast$\\{\scriptsize[0.001, 0.006]\;1/6}} \\
\addlinespace[2pt]Two effects $-$ free & \cellcolor{tabgreen}\makecell{+0.002\\{\scriptsize[$-$0.002, 0.006]\;0/9}} & \cellcolor{tabgreen}\makecell{+0.008$^\ast$\\{\scriptsize[0.003, 0.014]\;0/9}} &  & \cellcolor{tabgreen}\makecell{+0.006$^\ast$\\{\scriptsize[0.002, 0.010]\;1/6}} & \cellcolor{tabgreen}\makecell{+0.020$^\ast$\\{\scriptsize[0.013, 0.026]\;2/6}} &  \\
\midrule
\multicolumn{7}{l}{\emph{Fully connected}} \\
Two state-cond.\ effects & \cellcolor{tabgreen}0.659 & \cellcolor{tabred}0.658 & \cellcolor{tabred}\makecell{$-$0.001\\{\scriptsize[$-$0.002, 0.000]\;0/9}} & \cellcolor{tabred}0.554 & \cellcolor{tabgreen}0.555 & \cellcolor{tabgreen}\makecell{+0.001\\{\scriptsize[$-$0.001, 0.003]\;1/6}} \\
Free learner & \cellcolor{tabgreen}0.659 & \cellcolor{tabgreen}0.659 & \makecell{+0.000\\{\scriptsize[$-$0.000, 0.001]\;0/9}} & \cellcolor{tabgreen}0.551 & \cellcolor{tabgreen}0.551 & \makecell{$-$0.000\\{\scriptsize[$-$0.000, 0.000]\;0/6}} \\
\addlinespace[2pt]Two effects $-$ free & \makecell{+0.000\\{\scriptsize[$-$0.001, 0.001]\;0/9}} & \cellcolor{tabred}\makecell{$-$0.001\\{\scriptsize[$-$0.002, 0.001]\;0/9}} &  & \cellcolor{tabgreen}\makecell{+0.003$^\ast$\\{\scriptsize[0.002, 0.004]\;2/6}} & \cellcolor{tabgreen}\makecell{+0.004$^\ast$\\{\scriptsize[0.002, 0.006]\;3/6}} &  \\
\bottomrule
\end{tabular}}
\caption{Recursion control (final-node AUROC). Each edge model uses the parent's local risk $\sigma(b_p)$ (local) or the propagated $\hat r_p$ (propag.) and is trained with it. $\Delta$: propagated $-$ local, with 95\% bootstrap CI and the number of settings significant after Holm correction across the 15 settings of each system (4{,}000 draws on seed-averaged risks; none significant in the other direction). ``Two effects $-$ free'' compares the formulations. Green/red: higher/lower AUROC of each local--propagated pair, and positive/negative differences.}
\label{tab:recursion}
\end{table}


==> tables/qa_steps_main.tex <==
\begin{table*}[t]
\centering\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{In-domain} & \multicolumn{3}{c}{Transfer from MedQA} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
$\Delta$AUROC & Sequential & Fully conn. & Hierarchy & Sequential & Fully conn. & Hierarchy \\
\midrule
\makecell[l]{Receiver-text vs.\\Receiver Only} & \cellcolor{tabgreen}\makecell{+0.088$^\ast$\;{\footnotesize 9/9}\\{\footnotesize[0.062, 0.113]}} & \cellcolor{tabgreen}\makecell{+0.095$^\ast$\;{\footnotesize 9/9}\\{\footnotesize[0.080, 0.111]}} & \cellcolor{tabgreen}\makecell{+0.114$^\ast$\;{\footnotesize 6/6}\\{\footnotesize[0.087, 0.140]}} & \cellcolor{tabgreen}\makecell{+0.005\;{\footnotesize 4/6}\\{\footnotesize[$-$0.013, 0.022]}} & \cellcolor{tabred}\makecell{$-$0.002\;{\footnotesize 3/6}\\{\footnotesize[$-$0.014, 0.010]}} & \cellcolor{tabgreen}\makecell{+0.002\;{\footnotesize 2/3}\\{\footnotesize[$-$0.021, 0.026]}} \\
\makecell[l]{Interaction w/o parent\\state vs.\ Receiver-text} & \cellcolor{tabgreen}\makecell{+0.005\;{\footnotesize 6/9}\\{\footnotesize[$-$0.006, 0.016]}} & \cellcolor{tabgreen}\makecell{+0.018$^\ast$\;{\footnotesize 7/9}\\{\footnotesize[0.010, 0.026]}} & \cellcolor{tabgreen}\makecell{+0.005\;{\footnotesize 3/6}\\{\footnotesize[$-$0.008, 0.018]}} & \cellcolor{tabgreen}\makecell{+0.006\;{\footnotesize 3/6}\\{\footnotesize[$-$0.004, 0.015]}} & \cellcolor{tabgreen}\makecell{+0.013$^\ast$\;{\footnotesize 3/6}\\{\footnotesize[0.004, 0.022]}} & \cellcolor{tabgreen}\makecell{+0.020$^\ast$\;{\footnotesize 2/3}\\{\footnotesize[0.003, 0.039]}} \\
\makecell[l]{IE propagation vs.\\Receiver-text} & \cellcolor{tabgreen}\makecell{+0.019$^\ast$\;{\footnotesize 7/9}\\{\footnotesize[0.008, 0.032]}} & \cellcolor{tabgreen}\makecell{+0.018$^\ast$\;{\footnotesize 7/9}\\{\footnotesize[0.010, 0.026]}} & \cellcolor{tabred}\makecell{$-$0.004\;{\footnotesize 2/6}\\{\footnotesize[$-$0.019, 0.011]}} & \cellcolor{tabgreen}\makecell{+0.028$^\ast$\;{\footnotesize 5/6}\\{\footnotesize[0.016, 0.039]}} & \cellcolor{tabgreen}\makecell{+0.015$^\ast$\;{\footnotesize 6/6}\\{\footnotesize[0.006, 0.025]}} & \cellcolor{tabgreen}\makecell{+0.025$^\ast$\;{\footnotesize 2/3}\\{\footnotesize[0.008, 0.042]}} \\
\makecell[l]{IE propagation vs.\\PropUQ-MAS} & \cellcolor{tabgreen}\makecell{+0.071$^\ast$\;{\footnotesize 9/9}\\{\footnotesize[0.045, 0.096]}} & \cellcolor{tabgreen}\makecell{+0.077$^\ast$\;{\footnotesize 9/9}\\{\footnotesize[0.059, 0.094]}} & \cellcolor{tabgreen}\makecell{+0.083$^\ast$\;{\footnotesize 5/6}\\{\footnotesize[0.059, 0.107]}} & \cellcolor{tabred}\makecell{$-$0.007\;{\footnotesize 3/6}\\{\footnotesize[$-$0.025, 0.011]}} & \cellcolor{tabred}\makecell{$-$0.022$^\ast$\;{\footnotesize 1/6}\\{\footnotesize[$-$0.034, $-$0.009]}} & \cellcolor{tabgreen}\makecell{+0.018\;{\footnotesize 2/3}\\{\footnotesize[$-$0.008, 0.046]}} \\
\bottomrule
\end{tabular}}
\caption{Paired differences in final-node AUROC with the settings in which the first estimator is higher and the 95\% bootstrap CI (1{,}000 question-level resamples per setting); $^\ast$: CI excludes 0. Green: positive; red: negative. IE: interaction-effect; the interaction model without parent state adds a one-effect edge head on the full interaction to Receiver Only.}
\label{tab:qasteps}
\end{table*}


==> tables/qa_webqa.tex <==
\begin{table*}[tp]
\centering\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{Sequential} & \multicolumn{3}{c}{Fully connected} & \multicolumn{3}{c}{Hierarchy} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Estimator & NLL & Brier & AUROC & NLL & Brier & AUROC & NLL & Brier & AUROC \\
\midrule
\multicolumn{10}{l}{\emph{In-domain}: verbalized $u$} \\
Receiver-Only & 0.565 & 0.192 & 0.589 & 0.539 & 0.180 & 0.541 & 0.486 & 0.158 & 0.601 \\
Receiver-Text & 0.557 & 0.189 & 0.608 & \textbf{0.526} & \textbf{0.175} & \textbf{0.611} & \textbf{0.482} & \textbf{0.157} & 0.608 \\
Free Learner & \textbf{0.550} & \textbf{0.186} & \textbf{0.660} & 0.547 & 0.184 & 0.601 & 0.485 & 0.159 & 0.603 \\
Interaction-Effect Propagation & 0.554 & 0.187 & 0.659 & 0.546 & 0.184 & 0.600 & 0.483 & 0.158 & 0.605 \\
\cmidrule(lr){1-10}
PropUQ-MAS & 2.303 & 0.270 & 0.650 & 2.385 & 0.294 & 0.557 & 1.341 & 0.208 & \textbf{0.609} \\
\midrule
\multicolumn{10}{l}{\emph{In-domain}: MSP $u$} \\
Receiver-Only & 0.568 & 0.193 & 0.571 & 0.544 & 0.182 & 0.503 & 0.497 & 0.162 & 0.538 \\
Receiver-Text & 0.568 & 0.193 & 0.579 & \textbf{0.526} & \textbf{0.174} & \textbf{0.593} & 0.493 & \textbf{0.160} & 0.553 \\
Free Learner & \textbf{0.560} & \textbf{0.189} & 0.616 & 0.539 & 0.180 & 0.582 & 0.491 & \textbf{0.160} & 0.572 \\
Interaction-Effect Propagation & 0.561 & 0.190 & \textbf{0.617} & 0.539 & 0.180 & 0.582 & \textbf{0.489} & \textbf{0.160} & \textbf{0.576} \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.634 & 0.209 & 0.576 & 1.183 & 0.337 & 0.540 & 0.956 & 0.215 & 0.527 \\
\midrule
\multicolumn{10}{l}{\emph{In-domain}: entropy $u$} \\
Receiver-Only & 0.570 & 0.193 & 0.580 & 0.542 & 0.181 & 0.508 & 0.496 & 0.161 & 0.546 \\
Receiver-Text & 0.567 & 0.192 & 0.583 & \textbf{0.526} & \textbf{0.175} & \textbf{0.594} & 0.489 & 0.159 & 0.557 \\
Free Learner & \textbf{0.560} & \textbf{0.189} & \textbf{0.617} & 0.540 & 0.181 & 0.585 & 0.488 & 0.159 & 0.577 \\
Interaction-Effect Propagation & 0.561 & 0.190 & \textbf{0.617} & 0.540 & 0.181 & 0.584 & \textbf{0.486} & \textbf{0.158} & \textbf{0.578} \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.719 & 0.234 & 0.584 & 1.372 & 0.358 & 0.545 & 1.065 & 0.222 & 0.538 \\
\midrule
\multicolumn{10}{l}{\emph{Transfer from MedQA}: verbalized $u$} \\
Receiver-Only & 0.640 & 0.225 & 0.589 & 0.567 & 0.191 & 0.505 & 0.603 & 0.208 & 0.601 \\
Receiver-Text & 0.618 & 0.215 & 0.571 & 0.566 & 0.191 & 0.513 & 0.595 & 0.205 & \textbf{0.614} \\
Free Learner & \textbf{0.601} & \textbf{0.206} & 0.587 & 0.568 & 0.191 & 0.557 & 0.579 & 0.197 & 0.589 \\
Interaction-Effect Propagation & 0.611 & 0.211 & 0.590 & \textbf{0.564} & \textbf{0.190} & \textbf{0.561} & \textbf{0.573} & \textbf{0.195} & 0.591 \\
\cmidrule(lr){1-10}
PropUQ-MAS & 2.303 & 0.270 & \textbf{0.650} & 2.385 & 0.294 & 0.557 & 1.341 & 0.208 & 0.609 \\
\midrule
\multicolumn{10}{l}{\emph{Transfer from MedQA}: MSP $u$} \\
Receiver-Only & 0.646 & 0.228 & 0.571 & 0.570 & 0.192 & 0.503 & 0.610 & 0.212 & 0.532 \\
Receiver-Text & 0.603 & 0.210 & 0.536 & \textbf{0.555} & \textbf{0.187} & 0.503 & \textbf{0.588} & 0.205 & 0.513 \\
Free Learner & \textbf{0.581} & \textbf{0.199} & 0.566 & 0.575 & 0.189 & 0.534 & 0.631 & \textbf{0.193} & 0.545 \\
Interaction-Effect Propagation & 0.594 & 0.205 & 0.573 & 0.579 & 0.189 & 0.537 & 0.626 & 0.194 & \textbf{0.546} \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.634 & 0.209 & \textbf{0.576} & 1.183 & 0.337 & \textbf{0.540} & 0.956 & 0.215 & 0.527 \\
\midrule
\multicolumn{10}{l}{\emph{Transfer from MedQA}: entropy $u$} \\
Receiver-Only & 0.652 & 0.230 & 0.581 & 0.569 & 0.192 & 0.508 & 0.610 & 0.211 & 0.546 \\
Receiver-Text & 0.598 & 0.207 & 0.540 & \textbf{0.552} & \textbf{0.186} & 0.504 & \textbf{0.575} & 0.199 & 0.513 \\
Free Learner & \textbf{0.580} & \textbf{0.199} & 0.571 & 0.578 & 0.190 & 0.534 & 0.617 & \textbf{0.193} & 0.547 \\
Interaction-Effect Propagation & 0.585 & 0.201 & 0.581 & 0.590 & 0.192 & 0.535 & 0.622 & 0.195 & \textbf{0.548} \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.719 & 0.234 & \textbf{0.584} & 1.372 & 0.358 & \textbf{0.545} & 1.065 & 0.222 & 0.538 \\
\bottomrule
\end{tabular}}
\caption{Final-node error risk on WebQA in the three controlled systems: means over the three Qwen3 model sizes of the seed mean (3 seeds, 5 question-level folds; 500 test questions, at most 1 per setting dropped for an incomplete trace or missing $u$). Protocols, estimators and layout as in Table~\ref{tab:qa-gsm8k}. Transfer: estimators trained on MedQA traces of the same system and model. Bold: best value in each column of each block.}
\label{tab:qa-webqa}
\end{table*}


==> tables/scaling.tex <==
\begin{table*}[t]
\centering\footnotesize
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{\begin{tabular}{llcccccccc}
\toprule
 & & \multicolumn{2}{c}{Independent branches} & \multicolumn{2}{c}{Common root} & \multicolumn{2}{c}{Overlapping ancestry} & & \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Potentials & $k$ & NP & PME & NP & PME & NP & PME & MC ($10^3$) & NP / PME time (s) \\
\midrule
AppWorld & 2 & 0.042 & 0.000 & 0.041 & 0.000 & 0.048 & 0.005 & 0.003 & 5.3e-05 / 1.6e-04 \\
 & 4 & 0.039 & 0.000 & 0.043 & 0.001 & 0.052 & 0.006 & 0.003 & 8.7e-05 / 2.8e-04 \\
 & 8 & 0.043 & 0.000 & 0.046 & 0.002 & 0.064 & 0.009 & 0.005 & 1.7e-04 / 7.7e-04 \\
 & 16 & 0.045 & 0.000 & 0.047 & 0.003 & 0.079 & 0.014 & 0.004 & 3.1e-04 / 2.7e-02 \\
\midrule
WebArena & 2 & 0.055 & 0.000 & 0.056 & 0.001 & 0.066 & 0.004 & 0.007 & 6.4e-05 / 2.0e-04 \\
 & 4 & 0.066 & 0.000 & 0.069 & 0.000 & 0.076 & 0.003 & 0.005 & 1.1e-04 / 3.5e-04 \\
 & 8 & 0.078 & 0.000 & 0.091 & 0.001 & 0.099 & 0.003 & 0.007 & 3.2e-04 / 1.1e-03 \\
 & 16 & 0.094 & 0.000 & 0.099 & 0.002 & 0.113 & 0.004 & 0.008 & 3.7e-04 / 4.2e-02 \\
\bottomrule
\end{tabular}}
\caption{Width scaling on synthetic graphs whose conditionals are built from the learned state-supervised potentials (30 graphs per cell, edge effects scaled by $1/\sqrt{k}$ so the total interaction magnitude is fixed). Entries: mean $|r_{\mathrm{ref}}-r|$ at the sink, where the reference is structured exact inference, enumeration, or (overlapping ancestry, $k{=}16$, $2^{33}$ states) $10^6$-sample Rao--Blackwellised Monte Carlo. MC ($10^3$) and times are for the overlapping structure. NP keeps one scalar per node (about 2\,KB at $k{=}16$); PME and exact inference need $2^{k}$-entry tables at the sink (about 34\,MB at $k{=}16$).}
\label{tab:scaling}
\end{table*}


==> tables/steps.tex <==
\begin{table*}[t]
\centering\small
\setlength{\tabcolsep}{3.5pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{l}{\emph{In-domain}} \\
Step ($\Delta$AUROC) & Sequential ($n{=}9$) & Fully conn. ($n{=}9$) & Hierarchy ($n{=}6$) & & \\
\midrule
Receiver Only vs.\ raw uncertainty & \makecell{+0.005\\{\scriptsize[$-$0.000, +0.010]\;5/9}} & \makecell{$-$0.000\\{\scriptsize[$-$0.002, +0.002]\;5/9}} & \makecell{$-$0.000\\{\scriptsize[$-$0.002, +0.002]\;2/6}} & & \\
Receiver-text vs.\ Receiver Only & \makecell{+0.088$^\ast$\\{\scriptsize[+0.062, +0.113]\;9/9}} & \makecell{+0.095$^\ast$\\{\scriptsize[+0.080, +0.111]\;9/9}} & \makecell{+0.114$^\ast$\\{\scriptsize[+0.087, +0.140]\;6/6}} & & \\
Interaction vs.\ Receiver-text & \makecell{+0.005\\{\scriptsize[$-$0.006, +0.016]\;6/9}} & \makecell{+0.018$^\ast$\\{\scriptsize[+0.010, +0.026]\;7/9}} & \makecell{+0.005\\{\scriptsize[$-$0.008, +0.018]\;3/6}} & & \\
IE propagation vs.\ free learner & \makecell{+0.008$^\ast$\\{\scriptsize[+0.003, +0.014]\;9/9}} & \makecell{$-$0.001\\{\scriptsize[$-$0.002, +0.001]\;2/9}} & \makecell{$-$0.000\\{\scriptsize[$-$0.007, +0.007]\;4/6}} & & \\
IE propagation vs.\ local parent risk & \makecell{+0.012$^\ast$\\{\scriptsize[+0.006, +0.019]\;9/9}} & \makecell{$-$0.001\\{\scriptsize[$-$0.002, +0.000]\;3/9}} & \makecell{+0.000\\{\scriptsize[+0.000, +0.000]\;1/6}} & & \\
Free learner vs.\ local parent risk & \makecell{+0.006$^\ast$\\{\scriptsize[+0.002, +0.009]\;7/9}} & \makecell{+0.000\\{\scriptsize[$-$0.000, +0.001]\;5/9}} & \makecell{+0.000\\{\scriptsize[+0.000, +0.000]\;0/6}} & & \\
\midrule
IE propagation vs.\ Receiver-text & \makecell{+0.019$^\ast$\\{\scriptsize[+0.008, +0.032]\;7/9}} & \makecell{+0.018$^\ast$\\{\scriptsize[+0.010, +0.026]\;7/9}} & \makecell{$-$0.004\\{\scriptsize[$-$0.019, +0.011]\;2/6}} & & \\
IE propagation vs.\ PropUQ-MAS & \makecell{+0.071$^\ast$\\{\scriptsize[+0.045, +0.096]\;9/9}} & \makecell{+0.077$^\ast$\\{\scriptsize[+0.059, +0.094]\;9/9}} & \makecell{+0.083$^\ast$\\{\scriptsize[+0.059, +0.107]\;5/6}} & & \\
\midrule
\multicolumn{6}{l}{\emph{Transfer}} \\
Step ($\Delta$AUROC) & Sequential ($n{=}6$) & Fully conn. ($n{=}6$) & Hierarchy ($n{=}3$) & $\tau$ airline ($n{=}6$) & $\tau$ retail ($n{=}6$) \\
\midrule
Receiver Only vs.\ raw uncertainty & \makecell{+0.001\\{\scriptsize[$-$0.001, +0.003]\;3/6}} & \makecell{$-$0.000\\{\scriptsize[$-$0.002, +0.002]\;2/6}} & \makecell{+0.001\\{\scriptsize[$-$0.002, +0.004]\;1/3}} & \makecell{$-$0.089$^\ast$\\{\scriptsize[$-$0.116, $-$0.064]\;2/6}} & \makecell{$-$0.193$^\ast$\\{\scriptsize[$-$0.238, $-$0.146]\;0/6}} \\
Receiver-text vs.\ Receiver Only & \makecell{+0.005\\{\scriptsize[$-$0.013, +0.022]\;4/6}} & \makecell{$-$0.002\\{\scriptsize[$-$0.014, +0.010]\;3/6}} & \makecell{+0.002\\{\scriptsize[$-$0.021, +0.026]\;2/3}} & \makecell{$-$0.038$^\ast$\\{\scriptsize[$-$0.070, $-$0.005]\;1/6}} & \makecell{$-$0.081$^\ast$\\{\scriptsize[$-$0.145, $-$0.014]\;0/6}} \\
Interaction vs.\ Receiver-text & \makecell{+0.006\\{\scriptsize[$-$0.004, +0.015]\;3/6}} & \makecell{+0.013$^\ast$\\{\scriptsize[+0.004, +0.022]\;3/6}} & \makecell{+0.020$^\ast$\\{\scriptsize[+0.003, +0.039]\;2/3}} & \makecell{+0.074$^\ast$\\{\scriptsize[+0.050, +0.098]\;6/6}} & \makecell{+0.128$^\ast$\\{\scriptsize[+0.080, +0.175]\;5/6}} \\
IE propagation vs.\ free learner & \makecell{+0.020$^\ast$\\{\scriptsize[+0.013, +0.026]\;6/6}} & \makecell{+0.004$^\ast$\\{\scriptsize[+0.002, +0.006]\;5/6}} & \makecell{+0.003\\{\scriptsize[$-$0.006, +0.011]\;1/3}} & -- & -- \\
IE propagation vs.\ local parent risk & \makecell{+0.018$^\ast$\\{\scriptsize[+0.013, +0.023]\;6/6}} & \makecell{+0.001\\{\scriptsize[$-$0.001, +0.003]\;4/6}} & \makecell{+0.000\\{\scriptsize[+0.000, +0.000]\;1/3}} & -- & -- \\
Free learner vs.\ local parent risk & \makecell{+0.004$^\ast$\\{\scriptsize[+0.001, +0.006]\;4/6}} & \makecell{$-$0.000\\{\scriptsize[$-$0.000, +0.000]\;3/6}} & \makecell{+0.000\\{\scriptsize[+0.000, +0.000]\;0/3}} & -- & -- \\
\midrule
IE propagation vs.\ Receiver-text & \makecell{+0.028$^\ast$\\{\scriptsize[+0.016, +0.039]\;5/6}} & \makecell{+0.015$^\ast$\\{\scriptsize[+0.006, +0.025]\;6/6}} & \makecell{+0.025$^\ast$\\{\scriptsize[+0.008, +0.042]\;2/3}} & \makecell{+0.095$^\ast$\\{\scriptsize[+0.068, +0.122]\;6/6}} & \makecell{+0.155$^\ast$\\{\scriptsize[+0.110, +0.202]\;5/6}} \\
IE propagation vs.\ PropUQ-MAS & \makecell{$-$0.007\\{\scriptsize[$-$0.025, +0.011]\;3/6}} & \makecell{$-$0.022$^\ast$\\{\scriptsize[$-$0.034, $-$0.009]\;1/6}} & \makecell{+0.018\\{\scriptsize[$-$0.008, +0.046]\;2/3}} & \makecell{$-$0.065$^\ast$\\{\scriptsize[$-$0.096, $-$0.032]\;1/6}} & \makecell{$-$0.148$^\ast$\\{\scriptsize[$-$0.205, $-$0.091]\;1/6}} \\
\bottomrule
\end{tabular}}
\caption{Paired differences in final-node AUROC between rows of Table~\ref{tab:ladder}. Brackets: 95\% paired bootstrap CI (1{,}000 question-level resamples per setting, same items for both estimators); then the number of settings in which A exceeds B. $^\ast$: CI excludes 0. PRR differences, which follow the same pattern, are in Table~\ref{tab:prrsteps}.}
\label{tab:steps}
\end{table*}


==> tables/table1.tex <==
\begin{table*}[t]
\centering\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{Held-out GSM8K} & \multicolumn{3}{c}{Held-out MedQA} & \multicolumn{3}{c}{Held-out WebQA} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Estimator & Verb. & MSP & Entropy & Verb. & MSP & Entropy & Verb. & MSP & Entropy \\
\midrule
\multicolumn{10}{l}{\emph{Sequential}} \\
Receiver-Only & 0.557\rlap{$^{*}$} & \textbf{0.603} & \textbf{0.626} & 0.514\rlap{$^{*}$} & 0.436\rlap{$^{*}$} & 0.437\rlap{$^{*}$} & 0.589\rlap{$^{*}$} & 0.571 & 0.581 \\
Receiver-Text & 0.582\rlap{$^{*}$} & 0.587 & 0.605 & 0.505\rlap{$^{*}$} & 0.520 & 0.541 & 0.581\rlap{$^{*}$} & 0.527\rlap{$^{*}$} & 0.525\rlap{$^{*}$} \\
Free Learner & \textbf{0.634} & 0.596\rlap{$^{*}$} & 0.596\rlap{$^{*}$} & 0.555 & 0.543 & 0.565 & 0.617 & 0.563\rlap{$^{*}$} & 0.566\rlap{$^{*}$} \\
Interaction-Effect Propagation & \textbf{0.634} & \textbf{0.603} & 0.608 & 0.555 & 0.544 & 0.561 & 0.620 & 0.569 & 0.575 \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.605 & 0.544\rlap{$^{*}$} & 0.564\rlap{$^{*}$} & \textbf{0.576} & \textbf{0.564} & \textbf{0.572} & \textbf{0.650} & \textbf{0.576} & \textbf{0.584} \\
\midrule
\multicolumn{10}{l}{\emph{Fully connected}} \\
Receiver-Only & 0.544\rlap{$^{*}$} & 0.572 & 0.589 & 0.550 & 0.489\rlap{$^{*}$} & 0.474\rlap{$^{*}$} & 0.541 & 0.503\rlap{$^{*}$} & 0.508 \\
Receiver-Text & 0.550\rlap{$^{*}$} & 0.513\rlap{$^{*}$} & 0.525\rlap{$^{*}$} & 0.545\rlap{$^{*}$} & 0.529\rlap{$^{*}$} & 0.539\rlap{$^{*}$} & 0.510\rlap{$^{*}$} & 0.506\rlap{$^{*}$} & 0.506\rlap{$^{*}$} \\
Free Learner & 0.623 & 0.595 & 0.606 & 0.577 & \textbf{0.603} & 0.623 & 0.564 & \textbf{0.550} & \textbf{0.548} \\
Interaction-Effect Propagation & 0.618 & 0.593 & 0.605 & 0.577 & 0.601 & 0.622 & \textbf{0.566} & 0.549 & 0.546 \\
\cmidrule(lr){1-10}
PropUQ-MAS & \textbf{0.678}\rlap{$^{\dagger}$} & \textbf{0.652}\rlap{$^{\dagger}$} & \textbf{0.681}\rlap{$^{\dagger}$} & \textbf{0.582} & 0.602 & \textbf{0.635} & 0.557 & 0.540 & 0.545 \\
\midrule
\multicolumn{10}{l}{\emph{Hierarchy}} \\
Receiver-Only & 0.612\rlap{$^{*}$} & 0.651\rlap{$^{*}$} & 0.672\rlap{$^{*}$} & \textbf{0.587} & 0.396\rlap{$^{*}$} & 0.388\rlap{$^{*}$} & 0.601 & 0.539 & 0.546 \\
Receiver-Text & 0.646\rlap{$^{*}$} & 0.627\rlap{$^{*}$} & 0.642\rlap{$^{*}$} & 0.580 & 0.546\rlap{$^{*}$} & 0.564\rlap{$^{*}$} & 0.591 & 0.506\rlap{$^{*}$} & 0.499\rlap{$^{*}$} \\
Free Learner & 0.702\rlap{$^{*}$} & 0.736\rlap{$^{*}$} & 0.751\rlap{$^{*}$} & \textbf{0.587} & 0.608 & 0.622 & 0.594 & 0.553 & 0.554 \\
Interaction-Effect Propagation & \textbf{0.706} & 0.737 & 0.755 & \textbf{0.587} & 0.611 & \textbf{0.624} & 0.596 & \textbf{0.555} & \textbf{0.556} \\
\cmidrule(lr){1-10}
PropUQ-MAS & 0.648\rlap{$^{*}$} & \textbf{0.743} & \textbf{0.764} & 0.583 & \textbf{0.617} & 0.613 & \textbf{0.609} & 0.527 & 0.538 \\
\bottomrule
\end{tabular}}
\caption{AUROC of the final-node error risk under leave-one-dataset-out transfer in the three controlled systems. Every learned estimator is trained on the union of the training traces of two datasets (1{,}994--2{,}000 traces per setting) and evaluated on the test questions of the third (column group), which play no part in training, early stopping or calibration. Means over the three Qwen3 model sizes of the seed mean (3 seeds, 5 question-level folds; 1{,}319 GSM8K, 300 MedQA and 500 WebQA test questions, at most 8, 1 and 1 per setting dropped for an incomplete trace or missing $u$). Columns: held-out dataset and the node uncertainty $u_v$ that every estimator receives: Verb.\ ($1-{}$self-reported probability of being correct), MSP ($1-{}$geometric-mean probability of the visible tokens) or Entropy (mean top-20 token entropy over the visible tokens, divided by $\ln 20$). Learned rows share the encoder, folds and optimizer; PropUQ-MAS is training-free, so its values equal the in-domain ones. On held-out MedQA under MSP and Entropy, Receiver-Only, which sees only $u_v$ and the depth (the same for every final node), ranks the final nodes in the reverse order of $u_v$ (all three model sizes in the fully connected system and the hierarchy, 4B in the sequential system), hence values below 0.5. $^{*}$/$^{\dagger}$: Interaction-Effect Propagation is significantly higher/lower than that row (paired bootstrap over test questions, 1{,}000 draws shared by all rows; the 95\% interval of the difference of the model-size means excludes 0; no multiple-comparison correction). The interval covers test-question sampling, not training-seed variation (seed standard deviation of Interaction-Effect Propagation and Free Learner up to 0.020 per setting), so smaller marked differences, such as those to Free Learner, are not robust. Bold: best value in each column of each system.}
\label{tab:lodo}
\end{table*}


==> tables/variants.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{2.6pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{l}{\emph{In-domain}} \\
Model, $r_p$ & Sequential & Fully conn. & Hierarchy & & \\
\midrule
IE propagation, inferred & \textbf{0.655} & \textbf{0.658} & 0.612 & & \\
IE propagation, oracle & 0.809 & 0.368 & 0.528 & & \\
IE + receiver-text head, inferred & 0.654 & -- & \textbf{0.617} & & \\
\midrule
\multicolumn{6}{l}{\emph{Transfer}} \\
Model, $r_p$ & Sequential & Fully conn. & Hierarchy & $\tau$ airline & $\tau$ retail \\
\midrule
IE propagation, inferred & \textbf{0.569} & \textbf{0.555} & \textbf{0.524} & \textbf{0.521} & \textbf{0.564} \\
IE propagation, oracle & 0.726 & 0.535 & 0.566 & 0.626 & 0.686 \\
IE + receiver-text head, inferred & 0.562 & -- & 0.511 & 0.483 & 0.530 \\
\bottomrule
\end{tabular}}
\caption{Final-node AUROC of interaction-effect propagation with the parent risk $r_p$ inferred or set to the true parent error (oracle), and with an added receiver-text head (not run in the fully connected system). Oracle rows exclude the sequential MedQA 4B setting, for which no oracle predictions were computed, so in-domain sequential oracle rows average $n{=}8$ settings. The paired oracle$-$inferred difference for IE propagation is $+0.168$ in the sequential system and $+0.157$ under its transfer; in the fully connected system it is $-0.290$ and $-0.020$, because its end-to-end branches are mostly inverted (Table~\ref{tab:qabranch}). Bold: best inferred value in each column (oracle rows excluded).}
\label{tab:variants}
\end{table}

